Estimating Normalizing Constants for Log-Concave Distributions: Algorithms and Lower Bounds

Estimating the normalizing constant of an unnormalized probability distribution has important applications in computer science, statistical physics, machine learning, and statistics. In this work, we consider the problem of estimating the normalizing constant $Z=\int_{\mathbb{R}^d} e^{-f(x)}\,\mathrm{d}x$ to within a multiplication factor of $1 \pm \varepsilon$ for a $\mu$-strongly convex and $L$-smooth function $f$, given query access to $f(x)$ and $\nabla f(x)$. We give both algorithms and lowerbounds for this problem. Using an annealing algorithm combined with a multilevel Monte Carlo method based on underdamped Langevin dynamics, we show that $\widetilde{\mathcal{O}}\Bigl(\frac{d^{4/3}\kappa + d^{7/6}\kappa^{7/6}}{\varepsilon^2}\Bigr)$ queries to $\nabla f$ are sufficient, where $\kappa= L / \mu$ is the condition number. Moreover, we provide an information theoretic lowerbound, showing that at least $\frac{d^{1-o(1)}}{\varepsilon^{2-o(1)}}$ queries are necessary. This provides a first nontrivial lowerbound for the problem.

==> alt_upperbound.tex <==

\section{Alternative upper bound}

We need the following tail bound.
\begin{lem}\label{l:g-tail}
Suppose that $f:\R^d\to \R^d$ is a convex function, $\rh$ is a probability measure on $\R^d$ with  $\rh(\dx) = \rc{Z}e^{-\pa{\rc 2 \fc{\ve{x}^2}{\si^2}+f(x)}}\dx$, and $g(x) = {e^{\fc{\ve{x}^2}{2\si^2(1+\al^{-1})}}}$. 
Suppose $r_0\ge 2\si (1+\al) \sqrt{d}$ and let $r_0'=r_0-\si (1+\al) \sqrt{d}$. Then 
\begin{align}
\int_{\ve{x}\ge r_0} g(x) \rh(\dx)&\le 
2\al e^{\al d} e^{-\rc{2\si^2 (1+\al)}r_0^{\prime2}}
%\pa{1+\rc d} e^{-\pa{1+\rc d}r_0^{\prime2}}
%+ \fc{(d+1)^2 e^{-r_0^{\prime2}}\si^2}{4d\sqrt \pi r_0'}.
\end{align}
\end{lem}
\begin{proof}
By Lemma ??,
\begin{align}
\label{e:compare-tail}
\Pj_{x\sim \rh} (\ve{x}\ge r) \le \Pj_{x\sim N(0,\si^2)}(\ve{x}\ge r)
\end{align}
By the $\chi^2$ tail bound in~\cite{laurent2000adaptive}, 
\begin{align}
\label{e:chi-sq}
\Pj_{x\sim N(0,\si^2)}(\ve{x}^2\ge \si^2 (\sqrt d + \sqrt{2t})^2) 
\le 
\Pj_{x\sim N(0,\si^2)}(\ve{x}^2\ge \si^2 (d+2(\sqrt{dt}+t))) &\le e^{-t}.
\end{align}
Here, when $r=\si(\sqrt{d}+\sqrt{2t})$, we have $t=\rc 2\pa{\pf{r}{\si}-\sqrt d}^2
=\rc{2\si^2}\pa{r-\si\sqrt d}^2
$. 
Combining~\eqref{e:compare-tail} and~\eqref{e:chi-sq} we obtain that for $r\ge \sqrt d$, 
%We use a crude version of this bound:
\begin{align}
\Pj_{x\sim \rh}(\ve{x}\ge \si r)\le 
\Pj_{x\sim N(0,\si^2)}(\ve{x}\ge \si r) &\le e^{-\fc{1}{2\si^2}(r-\si \sqrt d)^2}.
\end{align}
For $r_0\ge d$, we calculate
\begin{align}
\int_{\ve{x}\ge r_0} g(x)\rh(\dx)
& = \int_{r_0}^{\infty} \ddd r \pa{e^{\fc{r^2}{2\si^2(1+\al^{-1})}}} \Pj_{x\sim \rh} (\ve{x}\ge r) \ud r\\
&= 
\int_{r_0}^{\infty}
\rc{\si^2(1+\al^{-1})}r
e^{\rc{2\si^2(1+\al^{-1})}r^2} 
\cdot 
e^{-\rc{2\si^2}(r-\si \sqrt d)^2}
\ud r\\
&=\int_{r_0}^{\infty}
\rc{\si^2(1+\al^{-1})}r
e^{-\rc{2\si^2(1+\al)}r^2 + \fc{\sqrt d}{\si} r - \fc d2}
\ud r\\
&=\int_{r_0}^{\infty}
\rc{\si^2(1+\al^{-1})}r
e^{-\rc{2\si^2(1+\al)}(r-\si(1+\al)\sqrt d)^2+\fc{\al d}2} \ud r\\
&=\int_{r_0-\si(1+\al)\sqrt d}^{\infty}
\fc{e^{\al d}}{\si^2(1+\al^{-1})}(r+\si(1+\al)\sqrt d)
e^{-\rc{2\si^2(1+\al)}r^2} \ud r\\
&\le\int_{r_0-\si(1+\al)\sqrt d}^{\infty}
\fc{2e^{\al d}}{\si^2(1+\al^{-1})}r
e^{-\rc{2\si^2(1+\al)}r^2} \ud r\\
&=2\al e^{\al d} e^{-\rc{2\si^2(1+\al)}r_0^{\prime2}}
\end{align}•
\end{proof}
\begin{lem}[Bias and variance calculation]\label{l:bias-var}
Suppose that $f:\R^d\to \R^d$ is a convex function, $\rh$ is a probability measure on $\R^d$ with  $\rh(\dx) = \rc{Z}e^{-\pa{\rc 2 \fc{\ve{x}^2}{\si^2}+f(x)}}\dx$, and $g(x) = e^{\fc{\ve{x}^2}{2\si^2(1+\al^{-1})}}$. 
Let $r_0=2\si (1+\al) \sqrt d$. Define
%2\si(1+\al)\pa{\sqrt d  + \sqrt{\ln \prc{\ep}}}$. 
\begin{align}
h(y) &=\begin{cases}
g(y) ,&\ve{y}\le r_0\\
e^{\fc{r_0^2}{2\si^2(1+\al^{-1})}}.
\end{cases}
\end{align}
Suppose that $W_2^2(\rh,\wt \rh)\le \de$. 
Let $L_h=\fc{2\al\sqrt d}{\si}e^{2\al(\al+1)d}$.
Then 
\begin{align}
\ab{\E_{x\sim \wt \rh}h(x)
- \E_{x\sim \rh}g(x)} &\le 2\al e^{-2d-\al d} + L_h \de\\
\Var_{\wt \rh}(h) &\le 2\Var_{\rh}(g) + 2L_h\de.
\end{align}
\end{lem}
\begin{proof}
\ul{Bias:}
By the triangle inequality,
\begin{align}
\ab{\E_{x\sim \wt\rh}h(x)
- \E_{x\sim \rh}g(x)}
&\le 
\ab{\E_{x\sim \rh}[h(x)-g(x)]}
+\ab{\E_{x\sim \wt \rh}h(x) - \E_{x\sim \rh} h(x)} .
\end{align}
To bound the first expression, we use the tail bound in Lemma~\ref{l:g-tail}.
\begin{align}
\ab{\E_{x\sim \rh}[h(x)-g(x)]}
&\le \int_{\ve{x}\ge r_0} g(x)\rh(\dx)
\le 2\al e^{\al d} e^{-\rc{2\si^2 (1+\al)}r_0^{\prime2}}
\le 2\al e^{\al d} e^{-2(1+\al)d}\le 2\al e^{-2d - \al d}.
\end{align}
To bound the second expression, we use the coupling and note that $h$ is Lipschitz with constant
\begin{align}
\max_{\ve{x}\le r_0} \ve{\nb g(x)}
& = \fc{r_0}{\si^2 (1+\al^{-1})}e^{\fc{r_0^2}{2\si^2(1+\al^{-1})}}
\le 
\fc{2\al \sqrt d}{\si} e^{\fc{4\si^2 (1+\al^2)d}{2\si^2(1+\al^{-1})}}
=\fc{2\al \sqrt d}{\si} 
e^{2\al(1+\al)d}=L_h.
\end{align}
By Kantorovich-Rubinstein duality, 
\begin{align}
\ab{\E_{x\sim \wt \rh}h(x) - \E_{x\sim \rh} h(x)}
& \le W_1(\rh, \wt \rh) L_h\le W_2(\rh, \wt \rh)L_h\le \de L_h.
\end{align}
Summing up the two inequalities gives the bound.

\ul{Variance:}
Let $\pi$ be an optimal coupling of $\rh$ and $\wt \rh$ achieving
\begin{align}
\int_{\R^d\times \R^d} \ve{x-y}^2 \pi(d(x,y))&=W_2^2(\rh, \wt \rh)\le \de^2.
\end{align}
Then
\begin{align}
\Var_{\wt \rh}(h) =
\E_{y\sim \wt \rh}\ba{h(y)^2 - \ba{\E_{x\sim \wt \rh}h(x)}^2}
&=
\E_{(x,y)\sim \pi} \ba{(h(y)-h(x)) + \pa{h(x)-\E_{x\sim \rh}h(x)}^2}\\
&\le 2\E_{(x,y)\sim \pi} [(h(y)-h(x))^2]
+ 2\Var_\rh(h)\\
&\le 2L_h\de + 2\Var_\rh(g)
\end{align}
where the last step follows from $h$ being $L_h$-Lipschitz and by the fact that thresholding a random variable cannot increase its variance. 
\end{proof}
\begin{lem}
Define $h_i$ for $g_i$ as in Lemma~\ref{l:bias-var}. Then ...
\end{lem}
\begin{proof}
Setting $\al = \rc{d}$, we get that $L_h = \fc{2}{\si_i \sqrt d} e^{2\pa{1+\rc d}}\le \fc{2e^4}{\si\sqrt d}$. Let $C_1=2e^4$. Setting $\de = \fc{C_1 \ep_1 \si_i}{\sqrt d}$, by Lemma~\ref{l:bias-var},
\begin{align}\label{e:bias-d}
\ab{\E_{\wt \rh_i} h_i - \E_{\rh_i}g_i} &\le \fc{2e^{-2d}}{d}+\fc{\ep_1}d\\
\label{e:var-d}
\Var_{\wt \rh} h&\le 2 \Var_\rh(g) + \fc{2\ep_1}d.
\end{align}
Note that for all $x$, $1\le h_i(x) \le  2e^{2\pa{1+\rc d}}\le 2e^4=C_1$, %, and $\E_{\rh_i}g_i\ge 1$.
and
\begin{align}\E_{\rh_i}g_i \le \E_{N\pa{0,\si_i^2}} g_i &= \fc{Z_i}{Z_{i+1}} =\pa{1+\rc d}^d\le e,
\end{align} by Harg\'e's Theorem. 

We carry out the concentration bounds in two steps: first, we show that with high probability, the estimate $\wh R_i$ of $R_i=\fc{Z_{i+1}}{Z_i}$ is within $\wt O(\ep)$, using the Chernoff bound. %can do Bernstein to get slightly better but I don't think it'll affect the final bound
The variance is actually $\wt O\pf{\ep^2}{d}$; however, we don't have control over the higher moments to prove that the estimate is within $\wt O\pf{\ep}{\sqrt d}$ with high probability. Secondly, using both the bound on the variance and high-probability bound of the magnitude of $\wh R_i-R_i$, we use Bernstein's inequality to prove that with high probability the product $\prod \wh R_i$ is close to $\prod R_i$ with relative error $1+\wt O(\ep)$. 

By the Chernoff bound, 
\begin{align}
\Pj\pa{
\ab{ \rc n \sumo jn h_i(X_j) - \EE_{\wt \rh}h_i}\ge \ep_2}
&\le e^{-\fc{n\ep_2^2}{2C^2}}.
\end{align}
%\fixme{Determine $t$}
Take $n\ge \fc{2C^2t^2}{\ep_2^2}\ln \pf{3M}{\de}$ to bound the probability by 
\begin{align}
\Pj\pa{
\ab{ \rc n \sumo jn h_i(X_j) - \EE_{\wt \rh}h_i}\ge \ep_2}
&\le \fc{\de}{3M}.
\end{align}
Using $\E_{\wt\rh_i}h_i\ge 1$ and~\eqref{e:bias-d}, 
\begin{align}
\Pj\pa{
\fc{\ab{ \rc n \sumo jn h_i(X_j) - \EE_{\wt \rh}h_i}}
{\E_{\wt\rh_i}h_i}\ge \ep_2 + \fc{2e^{-2d}}{d} + \fc{\ep_1}d} 
&\le \Pj\pa{
\ab{ \rc n \sumo jn h_i(X_j) - \EE_{\wt \rh}h_i}\ge \ep_2}
\le \fc{\de}{3M}.
\end{align}

Now let $\wt R_i = \E_{\wt\rh_i} h_i$ and let $\wh R_i= \rc n \sumo jn h_i(X_j)$ be our estimate. Let $D_i$ be such that $\wh R_i = \wt R_i (1+D_i)$. Above we established that $\Pj(|D_i|\ge \ep_2)\le \fc{\de}{3M}$. We also have by the variance bound~\eqref{e:var-d} and Lemma (variance lemma) that for some $C_2$,
\begin{align}
\Var_{\wt \rh_i}(h_i) &\le 2(e^{4\al^2d}-1)(\E_\rh g_i)^2 + \fc{2\ep}d
\le 2(e^{4/d}-1) e^2 + \fc{2\ep}d\le \fc{C_2}{d}.\\
\implies
\Var(D_i) 
&= \rc{\sqrt{n}} \Var_{x_1,\ldots, x_n\sim \wt \rh_i}\pa{\sumo jn h_i(x_j)}
\le \fc{C_2}{d\sqrt n}.
\end{align}
Let $\De = \fc{2^{-2d}}{d} + \fc{\ep}d$. 
We have
\begin{align}\label{e:prod-R}
\prodo i{M-1} R_i &= \prodo i{M-1} \wt R_i \prodo i{M-1} (1+D_i)\\
&\in \prodo i{M-1}\fc{Z_{i+1}}{Z_i} \prodo i{M-1} (1+D_i)
\ba{1-\De, 1+\De} = \fc{Z_M}{Z_1}\prodo i{M-1} (1+D_i) [e^{-2M\De}, e^{M\De}]
\end{align}
We now investigate the concentration of $\ln \prodo i{M-1} (1+D_i)$. Condition on each $|D_i|\le \ep_2$. Then by Taylor's Theorem, $\ln(1+D_i) = D_i - c_iD_i^2 $ for some $c_i\le 1$. Thus
\begin{align}
\log \prodo i{M-1} (1+D_i) &\in \ba{
\sumo i{M-1} D_i - \sumo i{M-1}D_i^2, 
\sumo i{M-1} D_i + \sumo i{M-1}D_i^2
}.
\end{align}
By Bernstein's inequality, \fixme{FIX: need to condition on $|D_i|\le \ep_2$, this is not 0-mean}
\begin{align}
\Pj\pa{
\ab{\sumo i{M-1} D_i}\ge \ep_3
}
&\le 2e^{-\fc{\ep_3^2}{2\pa{\fc{C_2}{d\sqrt n}+\rc3 \ep_2\ep_3}}}
\le e^{-\fc{\ep_3}{\ep_2}}
\end{align}
when $\fc{C_2}{d\sqrt n}\le \rc{6} \ep_2^2$ and $\ep_2\le \ep_3$.
Taking $\ep_3 = \ep_2\ln \pf{6}{\de}$, we get 
\begin{align}
\Pj\pa{
\ab{\sumo i{M-1} D_i}\ge \ep_3
}
&\le \fc{\de}{3}.
\end{align}
For the quadratic term, we note $\E D_i^2\le \fc{C_2}{d\sqrt n}$, and $\E[(D_i^2 - \E D_i^2)^2]\le \E D_i^4\le \E D_i^2$. %can have $\ep_1^2$ factor here
Hence we also have 
\begin{align}
\Pj\pa{\pa{\sumo i{M-1} D_i^2} - \fc{C_2M}{d\sqrt n}\ge \ep_3}&\le \fc{\de}{3}.
\end{align}
Then we get 
\begin{align}
\Pj\pa{\ab{\log \prodo i{M-1} (1+D_i)} \ge 2\ep_3 + \fc{C_2 M}{d\sqrt n}
}&\le \fc{2\de}3.
\end{align}
Combine with~\eqref{e:prod-R} and set constants appropriately.
\end{proof}
To finish, also include the bounds for the estimate of $Z_1$ and $Z_{M+1}/Z_M$.
\fixme{Add this.}

==> macros_stoc.tex <==
%LETTERS

%UPPERCASE
\newcommand{\sA}[0]{\mathscr{A}}
\newcommand{\cA}[0]{\mathcal{A}}
\newcommand{\A}[0]{\mathbb{A}}
\newcommand{\cB}[0]{\mathcal{B}}
\newcommand{\fB}[0]{\mathfrak{B}}
\renewcommand{\C}[0]{\mathbb{C}}
\newcommand{\sC}[0]{\mathcal{C}}%deprecated
\newcommand{\cC}[0]{\mathcal{C}}
\newcommand{\sD}[0]{\mathscr{D}}
\newcommand{\fD}[0]{\mathfrak{D}}
\newcommand{\mD}[0]{\mathfrak D}%deprecated
\newcommand{\cE}[0]{\mathscr{E}}%deprecated
\newcommand{\sE}[0]{\mathscr{E}}
%\newcommand{\E}[0]{\mathbb{E}}
%\newcommand{\EE}[0]{\mathop{\mathbb E}}
%\scalebox{1.25}{$\mathbb E$}}
\newcommand{\F}[0]{\mathbb{F}}
%\newcommand{\cF}[0]{\mathcal{F}}
\newcommand{\sF}[0]{\mathscr{F}}
%\newcommand{\G}[0]{\mathbb{G}}
\newcommand{\cG}[0]{\mathscr{G}}%deprecated.
\newcommand{\sG}[0]{\mathscr{G}}
\newcommand{\cH}[0]{\mathscr H}%deprecated
\newcommand{\sH}[0]{\mathscr H}
\newcommand{\Hq}[0]{\mathbb{H}}
\newcommand{\bfI}[0]{\mathbf{I}}
\newcommand{\I}[0]{\mathbb{I}}
\newcommand{\cI}[0]{\mathscr{I}}%deprecated
\newcommand{\sI}[0]{\mathscr{I}}
\newcommand{\cJ}[0]{\mathscr{J}}
\newcommand{\cK}[0]{\mathcal{K}}
\newcommand{\cL}[0]{\mathcal{L}}
\newcommand{\sL}[0]{\mathscr{L}}
\newcommand{\mM}[0]{\mathfrak{M}}
%\newcommand{\N}[0]{\mathbb{N}}
\newcommand{\fN}[0]{\mathfrak{N}}
\newcommand{\cP}[0]{\mathcal{P}}
\newcommand{\sP}[0]{\mathscr{P}}
\newcommand{\Pj}[0]{\mathbb{P}}
\newcommand{\mP}[0]{\mathfrak{P}}
\newcommand{\mQ}[0]{\mathfrak{Q}}
%!
\newcommand{\cO}[0]{\mathcal{O}}
\newcommand{\sO}[0]{\mathscr{O}}
\newcommand{\Q}[0]{\mathbb{Q}}
%\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\fR}[0]{\mathfrak{R}}
\newcommand{\bS}[0]{\mathbb{S}}
\newcommand{\T}[0]{\mathbb{T}}
\newcommand{\cT}[0]{\mathcal{T}}
\newcommand{\sT}[0]{\mathscr{T}}
\newcommand{\X}[0]{\mathfrak{X}}
\newcommand{\Z}[0]{\mathbb{Z}}
\newcommand{\one}[0]{\mathbbm{1}}
%lowercase
\newcommand{\mba}[0]{\mathbf{a}}%idele a
\newcommand{\ma}[0]{\mathfrak{a}}%ideal a
\newcommand{\mb}[0]{\mathfrak{b}}
%\newcommand{\mc}[0]{\mathfrak{c}}
\newcommand{\mfd}[0]{\mathfrak d}
\newcommand{\mf}[0]{\mathfrak{f}}
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\vi}[0]{\mathbf{i}}%vector i
\newcommand{\vj}[0]{\mathbf{j}}
\newcommand{\vk}[0]{\mathbf{k}}
\newcommand{\mm}[0]{\mathfrak{m}}%ideal m
\newcommand{\mfp}[0]{\mathfrak{p}}
\newcommand{\mq}[0]{\mathfrak{q}}
\newcommand{\mr}[0]{\mathfrak{r}}
\newcommand{\mv}[0]{\mathbf{v}}
\newcommand{\mx}[0]{\mathbf{x}}%idele x
\newcommand{\my}[0]{\mathbf{y}}
%More sequences of letters
\newcommand{\et}[0]{_{\text{\'et}}}
\newcommand{\Gm}[0]{\mathbb{G}_m}
\newcommand{\Fp}[0]{\mathbb{F}_p}
\newcommand{\fq}[0]{\mathbb{F}_q}
\newcommand{\fpb}[0]{\ol{\mathbb{F}_p}}
\newcommand{\fpt}[0]{\mathbb{F}_p^{\times}}
\newcommand{\fqt}[0]{\mathbb{F}_q^{\times}}
\newcommand{\Kt}[0]{K^{\times}}
\newcommand{\RP}[0]{\mathbb{R}P}
\newcommand{\qb}[0]{\ol{\mathbb{Q}}}
\newcommand{\qp}[0]{\mathbb{Q}_p}
\newcommand{\qpb}[0]{\ol{\mathbb{Q}_p}}
\newcommand{\ql}[0]{\mathbb Q_{\ell}}
\newcommand{\sll}[0]{\mathfrak{sl}}
\newcommand{\vl}[0]{V_{\ell}}
\newcommand{\zl}[0]{\mathbb Z_{\ell}}
\newcommand{\zp}[0]{\mathbb Z_{p}}
\newcommand{\zpz}[0]{\mathbb Z/p\mathbb Z}
%Shortcuts for greek letters
\newcommand{\al}[0]{\alpha}
\newcommand{\be}[0]{\beta}
\newcommand{\ga}[0]{\gamma}
\newcommand{\Ga}[0]{\Gamma}
\newcommand{\de}[0]{\delta}
\newcommand{\De}[0]{\Delta}
\newcommand{\ep}[0]{\varepsilon}
\newcommand{\eph}[0]{\frac{\varepsilon}{2}}
\newcommand{\ept}[0]{\frac{\varepsilon}{3}}
\newcommand{\ka}[0]{\kappa}
\newcommand{\la}[0]{\lambda}
\newcommand{\La}[0]{\Lambda}
\newcommand{\ph}[0]{\varphi}
\newcommand{\Ph}[0]{\Phi}
\newcommand{\rh}[0]{\rho}
\newcommand{\te}[0]{\theta}
\newcommand{\Te}[0]{\Theta}
\newcommand{\vte}[0]{\vartheta}
\newcommand{\om}[0]{\omega}
\newcommand{\Om}[0]{\Omega}
\newcommand{\si}[0]{\sigma}
\newcommand{\Si}[0]{\Sigma}
\newcommand{\ze}[0]{\zeta}

%SYMBOLS

%Shortcuts for symbols
\newcommand{\nin}[0]{\not\in}
\newcommand{\opl}[0]{\oplus}
\newcommand{\bigopl}[0]{\bigoplus}
\newcommand{\ot}[0]{\otimes}
\newcommand{\bigot}[0]{\bigotimes}
\newcommand{\sub}[0]{\subset}
\newcommand{\nsub}[0]{\not\subset}
\newcommand{\subeq}[0]{\subseteq}
\newcommand{\supeq}[0]{\supseteq}
\newcommand{\nsubeq}[0]{\not\subseteq}
\newcommand{\nsupeq}[0]{\not\supseteq}
%\newcommand{\nequiv}[0]{\not\equiv}
\newcommand{\bs}[0]{\backslash}
\newcommand{\iy}[0]{\infty}
\newcommand{\no}[0]{\trianglelefteq}%normal subgroup
\newcommand{\qeq}[0]{\stackrel?=}
\newcommand{\subsim}[0]{\stackrel{\sub}{\sim}}
\newcommand{\supsim}[0]{\stackrel{\supset}{\sim}}
\newcommand{\na}[0]{\nabla}
\newcommand{\mcv}[0]{*_-}
\newcommand{\dlim}[0]{\varinjlim}
\newcommand{\ilim}[0]{\varprojlim}
\newcommand{\gle}[0]{\begin{array}{c}
\ge\\
\le
\end{array}}
\newcommand{\lge}[0]{\begin{array}{c}
\le\\
\ge
\end{array}}
%\stackrel{-}{*}}%minus convoluion.

%COMMON TIME-SAVERS

%Fractions
\newcommand{\rc}[1]{\frac{1}{#1}}
\newcommand{\prc}[1]{\pa{\rc{#1}}}
\newcommand{\ff}[2]{\left\lfloor\frac{#1}{#2}\right\rfloor}
\newcommand{\cf}[2]{\left\lceil\frac{#1}{#2}\rceil\rfloor}
\newcommand{\fc}[2]{\frac{#1}{#2}}
\newcommand{\sfc}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\pf}[2]{\pa{\frac{#1}{#2}}}%Shortcut for fraction with parentheses
\DeclareRobustCommand{\stl}{\genfrac\{\}{0pt}{}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}%Partial derivatives
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\pdd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ddd}[1]{\frac{d}{d #1}}
\newcommand{\af}[2]{\ab{\fc{#1}{#2}}}
\newcommand{\ddt}[2]{\frac{d^2 #1}{d {#2}^2}}
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\pdxy}[3]{\frac{\partial^2 #1}{\partial {#2}\partial {#3}}}
\newcommand{\pl}[0]{\partial}
\newcommand{\nb}[0]{\nabla}
\newcommand{\onb}[0]{\ol{\nabla}}
\newcommand{\dy}{\ud y}
\newcommand{\dx}{\ud x}
\newcommand{\rdx}[0]{\mathrm dx} %no space version
\newcommand{\dt}{\ud t}
\newcommand{\dB}{\ud B}

%Arrows
\newcommand{\lar}[0]{\leftarrow}
\newcommand{\ra}[0]{\rightarrow}
\newcommand{\dra}[0]{\dashrightarrow}
\newcommand{\lra}[0]{\leftrightarrow}
\newcommand{\rra}[0]{\twoheadrightarrow}
\newcommand{\hra}[0]{\hookrightarrow}
\newcommand{\tra}[0]{\twoheadrightarrow}
\newcommand{\send}[0]{\mapsto}
\newcommand{\xra}[1]{\xrightarrow{#1}}
\newcommand{\xla}[1]{\xleftarrow{#1}}
\newcommand{\xhra}[1]{\xhookrightarrow{#1}}
\newcommand{\xlra}[1]{\xleftrightarrow{#1}}
\newcommand{\xrc}[0]{\xrightarrow{\cong}}
%\renewcommand{\cir}[0]{\circlearrowright}
\newcommand{\cil}[0]{\circlearrowleft}

%Brackets
\newcommand{\ab}[1]{\left| {#1} \right|}
\newcommand{\an}[1]{\left\langle {#1}\right\rangle}
\newcommand{\ba}[1]{\left[ {#1} \right]}
\newcommand{\bc}[1]{\left\{ {#1} \right\}}
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\braa}[1]{\langle\langle{#1}|}
\newcommand{\ce}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\fl}[1]{\left\lfloor {#1}\right\rfloor}
\newcommand{\ro}[1]{\left\lfloor {#1}\right\rceil}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\kett}[1]{|{#1}\rangle\rangle}
\newcommand{\bk}[2]{\langle{#1}|{#2}\rangle}
\newcommand{\braak}[2]{\langle\langle{#1}|{#2}\rangle\rangle}
\newcommand{\kbb}[1]{|{#1}\rangle\langle{#1}|}
\newcommand{\kb}[2]{|{#1}\rangle\langle{#2}|}
\newcommand{\kettb}[2]{|{#1}\rangle\rangle\langle\langle{#2}|}
\newcommand{\pa}[1]{\left( {#1} \right)}
\newcommand{\pat}[1]{\left( \text{#1} \right)}
\newcommand{\ve}[1]{\left\Vert {#1}\right\Vert}
\newcommand{\nv}[1]{\frac{#1}{\left\Vert {#1}\right\Vert}}
\newcommand{\nvl}[2]{\frac{#1}{\left\Vert {#1}\right\Vert_{#2}}}
\newcommand{\vvt}[1]{{#1}{#1}^\top}
\newcommand{\pvvt}[1]{\pa{#1}\pa{#1}^\top}
\newcommand{\vtv}[1]{{#1}^\top{#1}}
\newcommand{\pvtv}[1]{\pa{#1}^\top\pa{#1}}
\newcommand{\rb}[1]{\left.{#1}\right|}
\newcommand{\nl}[1]{\left\Vert #1 \right\Vert_{L^1}}
\newcommand{\ad}[0]{|\cdot|}
\newcommand{\ved}[0]{\ve{\cdot}}
\newcommand{\set}[2]{\left\{{#1}:{#2}\right\}}
\newcommand{\sett}[2]{\left\{\left.{#1}\right|{#2}\right\}}

%under and overlines, etc.
\newcommand{\ch}[1]{\check{#1}}
\newcommand{\dch}[1]{\check{\check{#1}}}
\newcommand{\olra}[1]{\overleftrightarrow{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ub}[2]{\underbrace{#1}_{#2}}
\newcommand{\ora}[1]{\overrightarrow{#1}}
\newcommand{\ura}[1]{\underrightarrow{#1}}
%\newcommand{\wt}[1]{\widetilde{#1}}
%\newcommand{\wh}[1]{\widehat{#1}}

%other
\newcommand{\fp}[1]{^{\underline{#1}}}%Falling power
\newcommand{\rp}[1]{^{\overline{#1}}}
\newcommand{\pp}[1]{^{(#1)}}
\newcommand{\sh}[0]{^{\sharp}}
\newcommand{\ri}[0]{\ddagger}%replace this with rosati involution
\newcommand{\bit}[0]{\{0,1\}}

%TEXT
\newcommand{\btih}[1]{\text{ by the induction hypothesis{#1}}}
\newcommand{\bwoc}[0]{by way of contradiction}
\newcommand{\by}[1]{\text{by~(\ref{#1})}}
\newcommand{\idk}[0]{{\color{red}I don't know.} }
\newcommand{\ore}[0]{\text{ or }}
\newcommand{\wog}[0]{ without loss of generality }
\newcommand{\Wog}[0]{ Without loss of generality }
\newcommand{\step}[1]{\noindent{\underline{Step {#1}:}}}
\newcommand{\prt}[1]{\noindent{\underline{Part {#1}:}}}
\newcommand{\tfae}[0]{ the following are equivalent}
\newcommand{\fabfm}[0]{for all but finitely many }

%FUNCTIONS
%Functions, etc.
\newcommand{\Abs}{(\text{Ab}/S)}
\newcommand{\abk}{(\text{Ab}/k)}
\newcommand{\abc}{(\text{Ab}/\C)}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\amax}{\operatorname{argmax}}
\newcommand{\amin}{\operatorname{argmin}}
\newcommand{\Ass}{\operatorname{Ass}}
\newcommand{\Art}{\operatorname{Art}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\avg}{\operatorname{avg}}
\newcommand{\bias}[0]{\operatorname{bias}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\Binom}{\operatorname{Binom}}
\newcommand{\Bl}[0]{\operatorname{Bl}}
\newcommand{\Br}{\operatorname{Br}}
\newcommand{\chr}{\operatorname{char}}
\newcommand{\cis}{\operatorname{cis}}
\newcommand{\cl}{\operatorname{Cl}}
%\newcommand{\Cl}{C}%changed notation%this is confusing
\newcommand{\Cl}{\operatorname{Cl}}
\newcommand{\Coh}{\operatorname{Coh}}
\newcommand{\Coinf}[0]{\operatorname{Coinf}}
\newcommand{\Coind}[0]{\operatorname{Coind}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\colim}{\operatorname{colim}}
\newcommand{\Comp}{\operatorname{Comp}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\oconv}{\ol{\conv}}
\newcommand{\Cor}{\operatorname{Cor}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\degs}[0]{\deg_{\text{s}}}%separable degree
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\depth}{\operatorname{depth}}
\newcommand{\Der}{\operatorname{Der}}
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\diam}{\operatorname{diam}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\Disc}{\operatorname{Disc}}%discrepancy
\newcommand{\disc}{\operatorname{disc}}%discriminant
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Ell}{\mathcal{E}{\rm{ll}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Ent}{\operatorname{Ent}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\err}{\operatorname{err}}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\pfcg}{(p\text{-FCGp}/k)}
\newcommand{\fcg}{(\text{FCGp}/k)}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\FS}{\operatorname{FS}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\gps}{(\text{Gp}/S)}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\Het}{H_{\text{\'et}}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Homeo}{\operatorname{Homeo}}
\newcommand{\chom}[0]{\mathscr{H}om}
\newcommand{\Homc}{\operatorname{Hom}_{\text{cont}}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\im}[0]{\text{im}}
\newcommand{\imp}[0]{\im^{\text{pre}}}
\newcommand{\Ind}[0]{\operatorname{Ind}}
\newcommand{\Inf}[0]{\operatorname{Inf}}
\newcommand{\inv}[0]{\operatorname{inv}}
\newcommand{\Isoc}[0]{\operatorname{Isoc}}
\newcommand{\Isog}[0]{\operatorname{Isog}}
\newcommand{\Isom}[0]{\operatorname{Isom}}
\newcommand{\KL}[0]{\operatorname{KL}}
\newcommand{\Jac}[0]{\operatorname{Jac}}
\newcommand{\li}[0]{\operatorname{li}}
\newcommand{\Li}[0]{\operatorname{li}}
\newcommand{\Lie}[0]{\operatorname{Lie}}
\newcommand{\Line}[0]{\operatorname{Line}}
\newcommand{\Lip}[0]{\operatorname{Lip}}
\newcommand{\lcm}[0]{\operatorname{lcm}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\Dmod}{\Mod_{W[F,V]}^{\text{fl}}}
\newcommand{\nil}[0]{\operatorname{nil}}
\newcommand{\nm}{\operatorname{Nm}}
\newcommand{\NS}{\operatorname{NS}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\PDer}{\operatorname{PDer}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Pico}{\operatorname{Pic}^{\circ}}
\newcommand{\Pois}{\operatorname{Pois}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\per}{\operatorname{per}}
\newcommand{\perm}{\operatorname{perm}}
\newcommand{\PrePer}{\operatorname{PrePer}}
\newcommand{\Prob}{\operatorname{Prob}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Prj}[0]{\textbf{Proj}}
\newcommand{\QCoh}{\operatorname{QCoh}}
\newcommand{\Rad}{\operatorname{Rad}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\red}{\operatorname{red}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Ric}{\operatorname{Ric}} %Ricci curvature
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\Scal}{\operatorname{Scal}} %Ricci curvature
\newcommand{\schs}{(\text{Sch}/S)}
\newcommand{\schk}{(\text{Sch}/k)}
\newcommand{\se}{\text{se}}
\newcommand{\srank}{\text{srank}}
\newcommand{\hse}{\wh{\text{se}}}
\newcommand{\Sel}{\operatorname{Sel}}
\newcommand{\sens}{\operatorname{sens}}
\newcommand{\Set}{(\text{Set})}
\newcommand{\sgn}{\operatorname{sign}}
%\newcommand{\sign}{\operatorname{sign}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Specf}[2]{\Spec\pa{\frac{k[{#1}]}{#2}}}
\newcommand{\rspec}{\ul{\operatorname{Spec}}}
\newcommand{\Spl}{\operatorname{Spl}}
\newcommand{\spp}{\operatorname{sp}}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\ssupp}{\operatorname{sing}\operatorname{supp}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\tor}{\operatorname{tor}}
\newcommand{\Tr}[0]{\operatorname{Tr}}
\newcommand{\tr}[0]{\operatorname{tr}}
\newcommand{\val}[0]{\text{val}}
\newcommand{\Var}[0]{\operatorname{Var}}
%\newcommand{\var}[0]{\text{var}}
\newcommand{\vcong}{\operatorname{vcong}}
\newcommand{\Vol}[0]{\text{Vol}}
\newcommand{\vol}[0]{\text{vol}}
\providecommand{\cal}[1]{\mathcal{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\providecommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\bb}[1]{\mathbb{#1}}

%Text super/subscripts
\newcommand{\abe}[0]{^{\text{ab}}}
\newcommand{\gal}[0]{^{\text{gal}}}%galois closure
\newcommand{\op}{^{\text{op}}}
\newcommand{\pre}[0]{^{\text{pre}}}
%\newcommand{\rd}[0]{_{\text{red}}}
\newcommand{\sep}[0]{^{\text{sep}}}
\newcommand{\tp}{^{\text{top}}}
\newcommand{\tors}{_{\text{tors}}}
\newcommand{\ur}[0]{^{\text{ur}}}
\newcommand{\urt}[0]{^{\text{ur}\times}}

%COMMUTATIVE DIAGRAMS

%Commutative diagram shortcuts
\newcommand{\commsq}[8]{\xymatrix{#1\ar[r]^-{#6}\ar[d]_{#5} &#2\ar[d]^{#7} \\ #3 \ar[r]^-{#8} & #4}}
%Makes a diagram like this
%1->2
%|    |
%3->4
%Arguments 5, 6, 7, 8 on arrows
%  6
%5  7
%  8
\newcommand{\pull}[9]{
#1\ar@/_/[ddr]_{#2} \ar@{.>}[rd]^{#3} \ar@/^/[rrd]^{#4} & &\\
& #5\ar[r]^{#6}\ar[d]^{#8} &#7\ar[d]^{#9} \\}
\newcommand{\back}[3]{& #1 \ar[r]^{#2} & #3}
%Syntax:\pull 123456789 \back ABC
%1=upper left-hand corner
%2,3,4=arrows from upper LH corner, going down, diagonal, right
%5,6,7=top row (6 on arrow)
%8,9=middle rows (on arrows)
%A,B,C=bottom row
%composition
\newcommand{\cmp}[9]{
\xymatrix{
#1 \ar[r]^{#4}{#5} \ar@/_2pc/[rr]^{#8}_{#9} & #2 \ar[r]^{#6}_{#7} & #3
}
}
\newcommand{\ctr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\ar[ld]_{#8}^{#9}\\
& #3 &
}
}
\newcommand{\ctrr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5} && #2\\
& #3 \ar[lu]_{#6}^{#7}\ar[ru]_{#8}^{#9}&
}
}

\newcommand{\ctri}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\\
& #3 \ar[ru]^{#8}_{#9}&
}
}
\newcommand{\rcommsq}[8]{\xymatrix{#1 &#2\ar[l]_-{#6} \\ #3 \ar[u]^{#5} & #4 \ar[u]_{#7}\ar[l]_-{#8}}}


%Arrow shortcuts
\newcommand{\ha}[1]{\ar@{^(->}[#1]}
\newcommand{\ls}[1]{\ar@{-}[#1]}
\newcommand{\sj}[1]{\ar@{->>}[#1]}
\newcommand{\aq}[1]{\ar@{=}[#1]}
\newcommand{\acir}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowright}}}
\newcommand{\acil}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowleft}}}
\newcommand{\ard}[1]{\ar@{.>}[#1]}
\newcommand{\mt}[1]{\ar@{|->}[#1]}
\newcommand{\inm}[1]{\ar@{}[#1]|-{\in}}
\newcommand{\inr}{\ar@{}[d]|-{\rotatebox[origin=c]{-90}{$\in$}}}
\newcommand{\inl}{\ar@{}[u]|-{\rotatebox[origin=c]{90}{$\in$}}}

%Other
%\newcommand{\set}[2]{\left.\left\{{#1}\right|{#2}\right\}}
%\newcommand{\sett}[2]{\left\{{#1}\left|{#2}\right\}\right.}

%SUMS, ETC.
\newcommand{\sumr}[2]{\sum_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%sum with 2 rows
\newcommand{\prr}[2]{\prod_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\maxr}[2]{\max_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\minr}[2]{\min_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\trow}[2]{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}
\newcommand{\seqo}[3]{\{#3\}_{#1=1}^{#2}}
\newcommand{\seqos}[3]{\{#3_#1\}_{#1=1}^{#2}}
\newcommand{\seqz}[3]{\{#3\}_{#1=0}^{#2}}
\newcommand{\seqzs}[3]{\{#3_#1\}_{#1=0}^{#2}}
\newcommand{\su}[0]{\sum_{n=0}^{\iy}}
\newcommand{\suo}[0]{\sum_{n=1}^{\iy}}
\newcommand{\sumo}[2]{\sum_{#1=1}^{#2}}
\newcommand{\sumz}[2]{\sum_{#1=0}^{#2}}
\newcommand{\prodo}[2]{\prod_{#1=1}^{#2}}
\newcommand{\prodz}[2]{\prod_{#1=0}^{#2}}
\newcommand{\oplo}[2]{\bigopl_{#1=1}^{#2}}
\newcommand{\cupo}[2]{\bigcup_{#1=1}^{#2}}
\newcommand{\capo}[2]{\bigcap_{#1=1}^{#2}}
\newcommand{\iiy}[0]{\int_0^{\infty}}
\newcommand{\iny}[0]{\int_{-\infty}^{\infty}}
\newcommand{\iiiy}[0]{\int_{-\infty}^{\infty}}%DEPRECATED
\newcommand{\sui}[0]{\sum_{i=1}^{n}}
\newcommand{\suiy}[0]{\sum_{i=1}^{\iy}}
\newcommand{\cui}[0]{\bigcup_{i=1}^n}
\newcommand{\suj}[0]{\sum_{j=1}^{n}}
\newcommand{\suij}[0]{\sum_{i,j}}
\newcommand{\limn}[0]{\lim_{n\to \infty}}

%MATRICES

%Matrices
\newcommand{\scoltwo}[2]{
\left(\begin{smallmatrix}
{#1}\\
{#2}
\end{smallmatrix}\right)}
\newcommand{\coltwo}[2]{
\begin{pmatrix}
{#1}\\
{#2}
\end{pmatrix}}
\newcommand{\colthree}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\colfour}[4]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}\\
{#4}
\end{pmatrix}
}
\newcommand{\cth}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\detm}[4]{
\ab{
\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}
\end{matrix}
}}
\newcommand{\sdetm}[4]{
\ab{
\begin{smallmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}
}}
\newcommand{\matt}[4]{
\begin{pmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{pmatrix}
}
\newcommand{\smatt}[4]{
\left(\begin{smallmatrix} 
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}\right)
}
\newcommand{\mattn}[9]{
\begin{pmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{pmatrix}
}

\newcommand{\bt}[2]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}
\end{matrix}
\right\}}
\newcommand{\bth}[3]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}\\
\text{#3}
\end{matrix}
\right\}}

\newcommand{\tcase}[4]{
\begin{cases}
#1 & #2\\
#3 & #4
\end{cases}}
\newcommand{\txcase}[4]{
\begin{cases}
#1 & \text{#2}\\
#3 & \text{#4}
\end{cases}}

\newcommand{\ifoth}[3]{
\begin{cases}
#1 & \text{if }#2\\
#3 & \text{otherwise}
\end{cases}}

%EQUATIONS
\newcommand{\beq}[1]{\begin{equation}\llabel{#1}}
\newcommand{\eeq}[0]{\end{equation}}
\newcommand{\bal}[0]{\begin{align*}}
\newcommand{\eal}[0]{\end{align*}}%this doesn't work; i don't know why
\newcommand{\ban}[0]{\begin{align}}
\newcommand{\ean}[0]{\end{align}}
\newcommand{\ig}[2]{\begin{center}\includegraphics[scale=#2]{#1}\end{center}}
\newcommand{\ign}[2]{\includegraphics[scale=#2]{#1}}

%COURSE-SPECIFIC

%measure theory, analysis
\newcommand{\am}[0]{(a.e., $\mu$)}
\newcommand{\ftla}[1]{\int e^{i\lambda\cdot x}{#1}\,d\lambda}
\newcommand{\lime}[0]{\lim_{\varepsilon\to 0}}

%number theory
\newcommand{\modt}[1]{\,(\text{mod}^{\times}\, {#1})}
%\newcommand{\tl}[0]{T_{\ell}}
 %multiplicative subgroup
\newcommand{\zmod}[1]{\Z/{#1}\Z}
\newcommand{\md}[1]{\,(\text{mod }#1)}
\newcommand{\ks}[1]{K(\sqrt{#1})}
\newcommand{\ksq}[1]{K(\sqrt{#1})/K}
\newcommand{\nksq}[1]{\nm_{K(\sqrt{#1})/K}(K(\sqrt{#1})^{\times})}
\newcommand{\mpp}[0]{\mP/\mfp}

%manifolds
\newcommand{\cvd}[0]{\frac{D}{\partial t}}
\newcommand{\cvs}[0]{\frac{D}{\partial s}}
\newcommand{\np}[1]{\nabla_{\pd{}{#1}}}

%algebraic geometry
\newcommand{\av}[0]{A^{\vee}}


%arithmetic combinatorics
\newcommand{\Deq}[1]{\Delta^{\times}_{#1}}

%modular forms
\newcommand{\GLAi}[0]{\text{GL}_2(\mathbb A)_{\infty}}

%noise sensitivity part iii essay
\newcommand{\Dict}[0]{\operatorname{\mathsf{Dict}}}
\newcommand{\Maj}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\MAJ}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\Parity}[0]{\operatorname{\mathsf{Parity}}}
\newcommand{\Tribes}[0]{\operatorname{\mathsf{Tribes}}}
\newcommand{\Ns}[0]{\operatorname{NS}}
\newcommand{\DT}[0]{\operatorname{\mathsf{DT}}}
\newcommand{\DNF}[0]{\operatorname{\mathsf{DNF}}}
\newcommand{\CNF}[0]{\operatorname{\mathsf{CNF}}}
\newcommand{\Circuit}[0]{\operatorname{\mathsf{Circuit}}}
\newcommand{\Ac}[0]{\mathsf{AC}}
\newcommand{\EB}[0]{\text{EB}}
%comp complexity
%complexity theory
\newcommand{\ACC}[0]{\operatorname{\mathsf{ACC}}}
\newcommand{\BPP}[0]{\mathsf{BPP}}
\newcommand{\BPTIME}[0]{\operatorname{\mathsf{BPTIME}}}
\newcommand{\CLIQUE}[0]{\operatorname{\mathsf{CLIQUE}}}
\newcommand{\EXP}[0]{\mathsf{EXP}}
\newcommand{\NEXP}[0]{\mathsf{NEXP}}
\newcommand{\NC}[0]{\operatorname{\mathsf{NC}}}
\newcommand{\NP}[0]{\operatorname{\mathsf{NP}}}
\newcommand{\NTIME}[0]{\operatorname{\mathsf{NTIME}}}
\newcommand{\msP}[0]{\operatorname{\mathsf{P}}}
\newcommand{\PCP}[0]{\operatorname{\mathsf{PCP}}}
\newcommand{\SAT}[0]{\mathsf{SAT}}
\newcommand{\SUBEXP}[0]{\mathsf{SUBEXP}}
\newcommand{\TIME}[0]{\operatorname{\mathsf{TIME}}}
\newcommand{\zz}{\textcircled{Z}}
%statistics
\newcommand{\hten}[0]{\widehat{\theta_n}}

%EDITING HELP
%blu: key idea or concept. red: unresolved issue/question. 
\newcommand{\blu}[1]{{\color{blue}#1}}
\newcommand{\grn}[1]{{\color{green}#1}}
\newcommand{\redd}[1]{{\color{red}#1}}
\newcommand{\pur}[1]{{\color{purple}#1}}
\newcommand{\oge}[1]{{\color{orange}#1}}
\newcommand{\concept}[1]{#1}
%\newcommand{\fixme}[1]{{\color{red}#1}}
\newcommand{\cary}[1]{{\color{purple}#1}}%deprecated
%short for commentary
%\newcommand{\llabel}[1]{\label{#1}\text{\fixme{\tiny#1}}}
\newcommand{\llabel}[1]{\label{#1}}
\newcommand{\nref}[1]{\ref{#1}}
%%%%%%%%%%%
%Use the above when working on the document, so labels will be displayed by their theorems, and you can write reminders to yourself. Switch to the below commands when publishing.
%%%%%%%%%%%
%\newcommand{\fixme}[1]{}
%\newcommand{\concept}[1]{{\color{blue}#1}}
%\newcommand{\llabel}[1]{\label{#1}}
%%%%%%%%%%%

\newcommand{\itag}[1]{\index{#1}[\##1]}
\newcommand{\ilbl}[1]{[#1]\index{#1}}
\newcommand{\iadd}[1]{\index{#1} #1}
\newcommand{\arxiv}[1]{\url{http://www.arxiv.org/abs/#1}}

%markup
\newcommand{\ivocab}[1]{\index{#1}\textbf{#1}}
\newcommand{\vocab}[1]{\textbf{#1}} %also index automatically.
\newcommand{\summq}[1]{\textbf{Summary Question: }#1}
\newcommand{\keypt}[1]{{\it #1}}
\newcommand{\subprob}[1]{\noindent\textbf{#1}\\}
\newcommand{\qatable}[1]{\begin{center}
    \begin{longtable}{ | p{5.5cm} | p{10cm} |}
#1
\end{longtable}
\end{center}}

%Page breaks in equations
\allowdisplaybreaks[2]

%SHA
\DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sh}{\mathord}{mcy}{"58} 

==> oldupperbound.tex <==
%\documentclass{amsart} 
%\renewcommand\baselinestretch{1.2}
%
%\usepackage{amsmath,amssymb}
%\usepackage{amsthm}
%\usepackage[alphabetic]{amsrefs}
%\usepackage{indentfirst}
%\usepackage{mathrsfs}
%\usepackage[notref, notcite]{showkeys}
%\usepackage{graphicx}
%\usepackage{hyperref}
%\usepackage{xcolor}
%\usepackage{fourier}
%\usepackage[margin=1.5in]{geometry}
%
%
%%\usepackage{lineno} 
%
%\usepackage{todonotes}
%\newcommand{\jlnotes}[1]{\todo[color=blue!35]{JL: #1}}
%\newcommand{\jl}[1]{\todo[inline,color=blue!35]{JL: #1}}
%
%% \numberwithin{equation}{section}
%
%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{estimate}[theorem]{Estimate}
%\newtheorem{prop}[theorem]{Proposition}
%\newtheorem{coro}[theorem]{Corollary}
%\newtheorem{conj}[theorem]{Conjecture}
%
%\theoremstyle{definition}
%\newtheorem{defn}[theorem]{Definition}
%\newtheorem*{notation}{Notation}
%\newtheorem{assump}{Assumption}
%\renewcommand{\theassump}{\Alph{assump}}
%
%\theoremstyle{remark}
%\newtheorem*{remark}{Remark}
%
%\DeclareMathOperator{\tr}{tr}
%\DeclareMathOperator{\pv}{p.v.}
%\DeclareMathOperator{\ran}{Ran}
%\DeclareMathOperator{\rank}{rank}
%\DeclareMathOperator{\dist}{dist}
%\DeclareMathOperator{\argmin}{arg min}
%\DeclareMathOperator{\spec}{spec}
%\DeclareMathOperator{\divop}{div}
%\DeclareMathOperator{\var}{Var}
%
%\newcommand{\thmref}[1]{Theorem~\ref{#1}}
%\newcommand{\corref}[1]{Corollary~\ref{#1}}
%\newcommand{\lemref}[1]{Lemma~\ref{#1}}
%\newcommand{\secref}[1]{\S\ref{#1}}
%\newcommand{\figref}[1]{Figure~\ref{#1}}
%
%\newcommand{\etc}{\textit{etc}.}
%\newcommand{\etal}{\textit{et al}}
%\newcommand{\ie}{\textit{i.e.}}
%\newcommand{\eg}{\textit{e.g.}}
%
%\newcommand{\ud}{\,\mathrm{d}}
%\newcommand{\rd}{\mathrm{d}}
%
%\newcommand{\RR}{\mathbb{R}}
%
%\newcommand{\NN}{\mathbb{N}}
%\newcommand{\ZZ}{\mathbb{Z}}
%\newcommand{\TT}{\mathbb{T}}
%\newcommand{\LL}{\mathbb{L}}
%\newcommand{\CC}{\mathbb{C}}
%\newcommand{\Or}{\mathcal{O}}
%\newcommand{\DD}{\mathcal{D}}
%
%\newcommand{\PP}{\mathbb{P}}
%\newcommand{\EE}{\mathbb{E}}
%
%\newcommand{\I}{\imath}
%
%\newcommand{\bd}[1]{\boldsymbol{#1}}
%\newcommand{\wt}[1]{\widetilde{#1}}
%\newcommand{\wh}[1]{\widehat{#1}}
%
%\newcommand{\dps}{\displaystyle}
%
%\IfFileExists{mathabx.sty}%
%  {\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}%
%   \DeclareFontShape{U}{mathx}{m}{n}{<->mathx10}{}%
%   \DeclareSymbolFont{mathx}{U}{mathx}{m}{n}%
%   \DeclareFontSubstitution{U}{mathx}{m}{n}%
%   \DeclareMathAccent{\widebar}{0}{mathx}{"73}%
%}{%
%  \PackageWarning{mathabx}{%
%    Package mathabx not available, therefore\MessageBreak substituting
%    widebar with overline\MessageBreak }%
%  \newcommand{\widebar}[1]{\overline{#1}}%
%}
%\newcommand{\wb}[1]{\widebar{#1}}
%
%\newcommand{\mc}[1]{\mathcal{#1}}
%\newcommand{\ms}[1]{\mathscr{#1}}
%\newcommand{\mf}[1]{\mathsf{#1}}
%
%\newcommand{\veps}{\varepsilon}
%\newcommand{\eps}{\epsilon}
%
%\newcommand{\abs}[1]{\lvert#1\rvert}
%\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
%\newcommand{\norm}[1]{\lVert#1\rVert}
%\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
%\newcommand{\average}[1]{\langle#1\rangle}
%\newcommand{\Average}[1]{\left\langle#1\right\rangle}
%\newcommand{\bra}[1]{\langle#1\rvert}
%\newcommand{\Bra}[1]{\left\langle#1\right\rvert}
%\newcommand{\ket}[1]{\lvert#1\rangle}
%\newcommand{\Ket}[1]{\left\lvert#1\right\rangle}
%\newcommand{\braket}[2]{\langle#1\mid#2\rangle}
%\newcommand{\Braket}[2]{\left\langle#1\mid#2\right\rangle}
%
%\renewcommand{\Re}{\mathfrak{Re}} 
%\renewcommand{\Im}{\mathfrak{Im}}
%
%% Local defined macros
%\renewcommand{\c}{\mathrm{c}}
%\newcommand{\x}{\mathrm{x}}
%\newcommand{\xc}{\mathrm{xc}}
%
%\title{}
%\author{Authors}
%\date{\today}
%\begin{document}
%\maketitle
%
%
%
%Given a $\mu$-convex and $L$-smooth function $f$, our goal is to estimate the 
%normalization constant 
%\begin{equation}
%  Z = \int_{\RR^d} e^{-f(x)} \ud x 
%\end{equation}
%within a multiplicative factor of $1 \pm \eps$ with probability more
%than $3/4$.
%
%
%
%\section{Upper bound}
%The algorithm we consider for estimating $Z$ is in the same spirit as
%the annealed importance sampling \cite{} in the statistic literature
%and thermodynamic integration \cite{} in the statistical physics
%literature. The method is based on defining a sequence of auxiliary
%distributions, given by the functions for $i = 1, 2, \ldots, M$
%\begin{equation}
%  f_i(x) = \frac{1}{2} \frac{\abs{x}^2}{\sigma_i^2} + f(x), 
%\end{equation}
%where $\sigma_1 \leq \sigma_2 \leq \cdots \leq \sigma_{M}$; for
%convenience of notation, we also define $\sigma_{M+1} = \infty$ so that
%$f_{M+1} = f$. Correspondingly we consider the sequence of distributions
%\begin{equation}
%  \rho_i(\rd x) = Z_i^{-1} e^{-f_i(x)} \ud x, 
%\end{equation}
%where $Z_i$ is the normalization constant
%\begin{equation}
%  Z_i = \int_{\RR^d} e^{-f_i(x)} \ud x. 
%\end{equation}
%The estimation of $Z$ is based on the identity 
%\begin{equation}\label{eq:estimateZ}
%  Z = Z_{M+1} = Z_1 \prod_{i=1}^M \frac{Z_{i+1}}{Z_i}. 
%\end{equation}
%
%
%In \eqref{eq:estimateZ}, we will approximate $Z_1$ by the normalization factor of the Gaussian distribution with variance $\sigma_1^2$. The approximation is guaranteed by the following lemma.  
%\begin{lemma}[Starting distribution] Let $\sigma_1 = \frac{\veps}{dL}$, we have 
%  \begin{equation}
%    (1 - \veps) \int_{\RR^d} e^{-\frac{1}{2} \frac{\abs{x}^2}{\sigma_1^2}} \ud x \leq Z_1 \leq \int_{\RR^d} e^{-\frac{1}{2} \frac{\abs{x}^2}{\sigma_1^2}} \ud x
%  \end{equation}
%\end{lemma}
%\begin{proof}
%  The upper bound is obvious since $f(x) \geq 0$ by our
%  assumption. For the lower bound of $Z_1$, note that
%  $f(x) \leq \frac{1}{2} L \abs{x}^2$, we have
%  \begin{equation}
%    \begin{aligned}
%      Z_1 & = \int_{\RR^d} e^{-f(x) - \frac{1}{2} \frac{\abs{x}^2}{\sigma_1^2}} \ud x \\
%      & \geq \int_{\RR^d} e^{ - \frac{1}{2} \bigl(L + \sigma_1^{-2} \bigr) \abs{x}^2} \ud x = \Bigl(2\pi \bigl( L + \sigma_1^{-2} \bigr)^{-1} \Bigr)^{d/2}
%    \end{aligned}
%  \end{equation}
%  Thus, 
%  \begin{equation}
%    \frac{Z_1}{(2\pi \sigma_1^2)^{d/2}} = \Bigl( 1 + \sigma_1^2 L  \Bigr)^{-d/2} \geq e^{-d\sigma_1^2 L / 2} 
%  \end{equation}
%  which is larger than $1 - \veps$ for $\sigma_1^2 = \frac{\veps}{dL}$.
%\end{proof}
%
%Next we consider the ratio $\frac{Z_{M+1}}{Z_M}$ in \eqref{eq:estimateZ} to determine the choice of $\sigma_M$. We have 
%\begin{equation}
%  \frac{Z_{M+1}}{Z_M} = \int  \exp\Biggl(\frac{\abs{x}^2}{2 \sigma_M^2}   \Biggr)\, \rho_M(\rd x) = \EE_{\rho_M}(g_M) 
%\end{equation}
%with 
%\begin{equation}
%  g_M =\exp\Biggl(\frac{\abs{x}^2}{2 \sigma_M^2}   \Biggr).
%\end{equation}
%Thus, the relative variance is given by 
%\begin{equation}
%  \begin{aligned}
%    \frac{\EE_{\rho_M}(g_M^2)}{\EE_{\rho_M} (g_M)^2}  = \EE_{\rho}
%    \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma_{M}^2}\Bigr)
%    \, \EE_{\rho} \exp\Bigl(\frac{1}{2} \frac{\abs{x}^2}{\sigma_{M}^2}  \Bigr). 
%  \end{aligned}
%\end{equation}
%
%\begin{lemma} Let $\sigma_M^2 = \frac{2d}{\mu}$, we have
%  \begin{equation*}
%    \EE_{\rho}
%    \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma_{M}^2}\Bigr)
%    \, \EE_{\rho} \exp\Bigl(\frac{1}{2} \frac{\abs{x}^2}{\sigma_{M}^2}  \Bigr)
%    \leq \exp \Bigl( \frac{4d}{\mu\sigma_M^4}  \Bigr) = \exp \Bigl( \frac{\mu}{d}  \Bigr). 
%  \end{equation*}
%
%\end{lemma}
%
%\begin{proof}
%  Define
%  \begin{equation*}
%    h(t) := \EE_{\rho} e^{-t\abs{x}^2} \EE_{\rho} e^{t\abs{x}^2}. 
%  \end{equation*}
%  We have
%  \begin{equation*}
%    \begin{aligned}
%      \frac{h'(t)}{h(t)} & = \dfrac{\EE_{\rho} \Bigl( \abs{x}^2
%        e^{t\abs{x}^2} \Bigr)} {\EE_{\rho} e^{t\abs{x}^2}} -
%      \dfrac{\EE_{\rho} \Bigl( \abs{x}^2 e^{-t\abs{x}^2} \Bigr)}
%      {\EE_{\rho} e^{-t\abs{x}^2}}  \\
%      & = \int_{-t}^t v'(s)\ud s, 
%    \end{aligned}
%  \end{equation*}
%  where
%  \begin{equation*}
%    v(s) = \dfrac{\EE_{\rho} \Bigl( \abs{x}^2
%      e^{s\abs{x}^2} \Bigr)} {\EE_{\rho} e^{s\abs{x}^2}},. 
%  \end{equation*}
%  Thus
%  \begin{equation*}
%    \begin{aligned}
%      v'(s) & = \dfrac{\EE_{\rho} \Bigl( \abs{x}^4 e^{s\abs{x}^2}
%        \Bigr)\EE_{\rho} e^{s\abs{x}^2} - \biggl(\EE_{\rho} \Bigl(
%        \abs{x}^2
%        e^{s\abs{x}^2} \Bigr)\biggr)^2 } {\biggl(\EE_{\rho} e^{s\abs{x}^2}\biggr)^2}\\
%      & = \var_{\rho_s} \bigl( \abs{x}^2 \bigr), 
%    \end{aligned}
%  \end{equation*}
%  where $\rho_s$ is a distribution with $\frac{\ud\rho_s}{\ud\rho} \propto e^{s\abs{x}^2}$. Since $\rho$ is strongly-concave with convexity $\mu$, $\rho_s$ satisfies the Poincar\'e inequality with constant $1/ (\mu - 2s) \leq 2/\mu$ for $s \leq \frac{1}{4} \mu$, thus
%  \begin{equation}
%    \var_{\rho_s} \bigl( \abs{x}^2 \bigr) \leq \frac{8}{\mu} \EE_{\rho_s} \bigl( \abs{x}^2 \bigr) \leq \frac{16}{\mu} d,
%  \end{equation}
%  where the last inequality follows from the concentration property of logconcave distribution.
%
%  Therefore,
%  \begin{equation*}
%    \begin{aligned}
%      \ln h\bigl(\frac{1}{2\sigma_M^2}\bigr) & = \ln h(0) + \int_0^{1/(2\sigma_M^{2})} \frac{h'(t)}{h(t)} \ud t \\
%      & \leq \int_0^{1/(2\sigma_M^{2})} \frac{32}{\mu} d t \ud t \\
%      & = \frac{4d}{\mu\sigma_M^4} 
%    \end{aligned}
%  \end{equation*}
%  and we arrive at
%  \begin{equation*}
%    \EE_{\rho}
%    \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma_{M}^2}\Bigr)
%    \, \EE_{\rho} \exp\Bigl(\frac{1}{2} \frac{\abs{x}^2}{\sigma_{M}^2}  \Bigr)
%    \leq \exp \Bigl( \frac{4d}{\mu\sigma_M^4}  \Bigr).
%  \end{equation*}
%  The choice $\sigma_M^2 = 2 d / \mu$ (which satisfies also $1/ (2 \sigma_M^2) \leq \mu / 4$) guarantees the desired estimate.  
%\end{proof}
%
%
%
%Let us now consider the ratio $\frac{Z_{i+1}}{Z_i}$ in
%\eqref{eq:estimateZ}. Notice that
%\begin{equation}
%  \frac{Z_{i+1}}{Z_i} = \int  \exp\Biggl(\frac{1}{2}\Bigl(\frac{1}{\sigma_i^2} - \frac{1}{\sigma_{i+1}^2}\Bigr) \abs{x}^2 \Biggr)\, \rho_i(\rd x) = \EE_{\rho_i}(g_i) 
%\end{equation}
%where
%\begin{equation}
%  g_i = \exp\Biggl(\frac{1}{2}\Bigl(\frac{1}{\sigma_i^2} - \frac{1}{\sigma_{i+1}^2}\Bigr) \abs{x}^2 \Biggr).
%\end{equation}
%
%To bound the variance of $g_i$ under the distribution $\rho_i$, we calculate 
%\begin{equation}
%  \frac{\EE_{\rho_i}(g_i^2)}{\EE_{\rho_i} (g_i)^2} =
%  \dfrac{\EE_{\rho} \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma_{i}^2}\Bigr)
%  \, \EE_{\rho} \exp\Bigl(\frac{1}{2} \frac{\abs{x}^2}{\sigma_{i}^2} - \frac{\abs{x}^2}{\sigma_{i+1}^2} \Bigr)}{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma_{i+1}^2}\Bigr)\biggr)^2}
%\end{equation}
%Let $\sigma^2 = \sigma_{i+1}^2$ and $\sigma_i^2 = \sigma^2 / ( 1 + \alpha)$, we have 
%\begin{equation}
%    \frac{\EE_{\rho_i}(g_i^2)}{\EE_{\rho_i} (g_i)^2} = 
%    \dfrac{\EE_{\rho} \exp\Bigl(-\frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)
%  \, \EE_{\rho} \exp\Bigl(-\frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)}{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\biggr)^2}. 
%\end{equation}
%The next lemma gives an upper bound for the right hand side as $\exp(4 \alpha^2 d)$, thus suggests the choice $\alpha = \Theta(1/d)$. 
%
%\begin{lemma}
%  Let $\rho$ be a logconcave distribution,  for $\alpha \leq \frac{1}{2}$, we have
%  \begin{equation}
%    \dfrac{\EE_{\rho} \exp\Bigl(-\frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)
%      \, \EE_{\rho} \exp\Bigl(-\frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)}{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\biggr)^2}
%    \leq \exp \bigl( 4 \alpha^2 d \bigr) 
%  \end{equation}
%\end{lemma}
%
%The proof follows along similar lines as the previous Lemma. 
%
%\begin{proof}
%  Define 
%  \begin{equation*}
%    h(\alpha) :=     \EE_{\rho} \exp\Bigl(-\frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)
%      \, \EE_{\rho} \exp\Bigl(-\frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr).
%  \end{equation*}
%  It follows then 
%  \begin{equation*}
%    \begin{aligned}
%      \frac{h'(\alpha)}{h(\alpha)} & = - \frac{1}{2\sigma^2} \left( \dfrac{\EE_{\rho} \Bigl( \abs{x}^2 \exp\Bigl(-\frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr) \Bigr)}{\EE_{\rho} \exp\Bigl(-\frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)} - \dfrac{\EE_{\rho} \Bigl(\abs{x}^2 \exp\Bigl(-\frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\Bigr)}{\EE_{\rho} \exp\Bigl(-\frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)} \right) \\
%      & = - \frac{1}{2\sigma^2} \int_{1-\alpha}^{1+\alpha} v'(t) \ud t 
%    \end{aligned}
%  \end{equation*}
%  where $v(t)$ is defined as 
%  \begin{equation*}
%    v(t) := \dfrac{\EE_{\rho} \Bigl( \abs{x}^2 \exp\Bigl(-\frac{t}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr) \Bigr)}{\EE_{\rho}  \exp\Bigl(-\frac{t}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)}. 
%  \end{equation*}
%  Explicit calculation gives 
%  \begin{equation*}
%    \begin{aligned}
%      v'(t) & = - \frac{1}{2\sigma^2} \dfrac{\EE_{\rho} \Bigl(
%        \abs{x}^4 \exp\Bigl(-\frac{t}{2}
%        \frac{\abs{x}^2}{\sigma^2}\Bigr) \Bigr)
%        \EE_{\rho}  \exp\Bigl(-\frac{t}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr) - \biggl(\EE_{\rho} \Bigl( \abs{x}^2 \exp\Bigl(-\frac{t}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr) \Bigr) \biggr)^2}{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{t}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\biggr)^2} \\
%      & = - \frac{1}{2\sigma^2} \var_{\rho_t}(\abs{x}^2)
%    \end{aligned}
%  \end{equation*}
%  here $\rho_t$ is the distribution given by 
%  \begin{equation*}
%    \frac{\ud \rho_t}{\ud \rho} \propto \exp\Bigl(-\frac{t}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr). 
%  \end{equation*}
%  By the Poincar\`e inequality and concentration property of strongly log-concave measure 
%  \begin{equation*}
%    \var_{\rho_t}(\abs{x}^2) \leq \frac{4\sigma^2}{t} \EE_{\rho_t} \abs{x}^2 
%    \leq 8\frac{\sigma^4}{t^2} d. 
%  \end{equation*}
%  Therefore, we arrive at the inequality 
%  \begin{equation*}
%    \begin{aligned}
%      \dfrac{h'(\alpha)}{h(\alpha)} & = \frac{1}{4\sigma^4} \int_{1-\alpha}^{1+\alpha} \var_{\rho_t} (\abs{x}^2)  \ud t \\
%      & \leq 2d \int_{1-\alpha}^{1+\alpha} \frac{1}{t^2} \ud t \\
%      & = 2d \Bigl( \frac{1}{1-\alpha} - \frac{1}{1+\alpha} \Bigr) \\
%      & \leq 8 d \alpha.
%    \end{aligned}
%  \end{equation*}
%  Therefore 
%  \begin{equation*}
%    \ln h(\alpha) - \ln h(0) = \int_0^{\alpha} \dfrac{h'(\alpha)}{h(\alpha)} \ud \alpha  \leq 4 d \alpha^2. 
%  \end{equation*}
%  Thus, we arrive that 
%  \begin{equation*}
%    \frac{h(\alpha)}{h(0)} \leq e^{4d \alpha^2},  
%  \end{equation*}
%  which is the desired inequality by the definition of $h$.
%\end{proof}
%
%
%
%
%\begin{lemma}
%  Let $\rho$ be a strongly-logconcave distribution with $\mu$-convex
%  and $L$-smooth, for $\alpha \leq \frac{1}{2}$, we have
%  \begin{equation}
%    \dfrac{\EE_{\rho} \exp\Bigl(-\frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)
%      \, \EE_{\rho} \exp\Bigl(-\frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)}{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\biggr)^2}
%    \leq \exp \biggl( \frac{ 4 \alpha^2 d \log(1/\veps)^2}{\mu \sigma^2} \biggr)
%  \end{equation}
%  \jl{need to check to make sure; especially as it  involves cutting the distribution which induces another $(1 - \veps)$ factor error?}
%\end{lemma}
%
%\jl{useful fact for proving the above}
%Let $X \in \RR^d$ a random variable distributed from a logconcave
%distribution with $\EE(\abs{X}^2) = R^2$. Restricted the support of
%$X$ to a ball with radius $2R \log (1/ \veps)$ captures at least
%$1 - \veps / 2$ fraction of the mass.
%\bigskip 
%
%
%% Case 1. $\sigma^2 \lesssim 1$
%% \begin{equation}
%% \dfrac{\Bigl( L  + \frac{1}{\sigma^2} \Bigr)^{d}}{\Bigl( \mu  + \frac{1+\alpha}{\sigma^2} \Bigr)^{d/2} \Bigl( \mu + \frac{1-\alpha}{\sigma^2} \Bigr)^{d/2}} \lesssim \dfrac{ (1 / \sigma^2)^d}{\bigl((1 - \alpha^2)/\sigma^4\bigr)^{d/2}} = \frac{1}{(1-\alpha^2)^{d/2}}
%% \end{equation}
%% If we choose $\alpha \sim \frac{1}{d}$: variance $\Or(1)$, number of
%% phases $\Or(d)$. \textcolor{red}{Cost per sample $\sim d^{1/2}\eps^{-1}$: need to establish the estimate} 
%
%% Case 2. $\sigma^2 \gg 1$; not sure whether it is needed.  We can take
%% $\alpha \sim \frac{\sigma^2}{d}$ while maintaining the variance being $\Or(1)$. 
%
%
%
%
%\bigskip 
%
%
%
%Fixing $\sigma$ and $\alpha$, we need to estimate the expectation of 
%\begin{equation}\label{eq:gdef}
%  g = \exp \biggl( \frac{1}{2} \frac{\alpha}{\sigma^2} \abs{x}^2  \biggr)
%\end{equation}
%under the distribution proportional to 
%\begin{equation}\label{eq:gdefdist}
%  \exp\biggl( - \frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2} - f(x)  \biggr) \ud x.
%\end{equation}
%By the above choice of $\alpha$ and $\sigma^2$, we have
%$\frac{1}{d} \lesssim \frac{\alpha}{\sigma^2} \lesssim \frac{1}{\veps}$.  The tricky
%point is that this function is not globally Lipschitz, and thus one
%cannot immediately rely on the convergence of sampling in Wasserstein
%metric. In particular, to obtain an estimate of MSE, we need a moment
%bound of the empirical distribution, denoted as $\rho^{(n)}$ ($n$ is the
%number of sampling steps), as
%\begin{equation}
%  \EE_{\rho^{(n)}} (g^2) / \bigl(\EE_{\rho^{(n)}} g \bigr)^2.
%\end{equation}
%
%
%
%
%For simplicity, let us not use warm start and assume we start the
%underdamped Langevin sampler at $X = 0$ for a log-concave distribution
%that is $\mu$-convex and $L$-smooth, denoted by
%$\rd \rho = Z^{-1} e^{-f(x)}\ud x$.
%
%\jl{should be a stand-alone result}
%
%
%
%
%Let $\wt{X}^{(k)}$ be iid random variables with distribution $\wt{\rho}$, which is an approximation of $\rho$. We would like to control for $g(x) = \exp\bigl(a\abs{x}^2 / 2 \bigr)$
%
%\begin{lemma}
%  Let $\wt{X}^{(k)}$ be iid random variables with distribution
%  $\wt{\rho}$.  Let $g(x) = \exp\bigl(a\abs{x}^2 / 2 \bigr)$, ...
%  \begin{multline}\label{eq:msebound}
%    \EE_{\wt{\rho}} \Biggl[   \frac{1}{K} \sum_{k=1}^K g(\wt{X}^{(k)}) - \EE_{\rho} g \Biggr]^2 \leq (\EE_{\rho} g)^2 \Bigl( \frac{1}{K} \frac{\var_{\rho} g}{(\EE_{\rho} g)^2} + \frac{4}{K} \frac{\max \bigl\{\EE_{\wt{\rho}} \abs{g \nabla g}^2, \EE_{\rho} \abs{g \nabla g}^2 \bigr\}^{1/2}}{(\EE_{\rho} g)^2} W_2 (\wt{\rho}, \rho)  \\ 
%    + \frac{1}{K} \dfrac{\EE_{\wt{\rho}} g + \EE_{\rho} g}{(\EE_{\rho} g)^2} \max \bigl\{\EE_{\wt{\rho}} \abs{\nabla g}^2, \EE_{\rho} \abs{\nabla g}^2 \bigr\}^{1/2}W_2 (\wt{\rho}, \rho) +   \frac{\max \bigl\{\EE_{\wt{\rho}} \abs{\nabla g}^2, \EE_{\rho} \abs{\nabla g}^2 \bigr\}}{(\EE_{\rho} g)^2} W_2 (\wt{\rho}, \rho)^2  \Bigr) 
%  \end{multline}
%\end{lemma} 
%
%\jl{not sure how to gain another factor of $d$ from the last term, besides $\veps^2$ from Wasserstein distance.} 
%
%\begin{proof} First note that 
%\begin{equation*}
%  \begin{aligned}
%    \EE_{\wt{\rho}} \Biggl[   \frac{1}{K} \sum_{k=1}^K g(\wt{X}^{(k)}) - \EE_{\rho} g \Biggr]^2 & = \EE_{\wt{\rho}} \Biggl[   \frac{1}{K} \sum_{k=1}^K g(\wt{X}^{(k)}) - \EE_{\wt{\rho}} g \Biggr]^2
%  + \bigl( \EE_{\wt{\rho}} g - \EE_{\rho} g \bigr)^2 \\
%  & = \frac{1}{K} \var_{\wt{\rho}} g
%  + \bigl( \EE_{\wt{\rho}} g - \EE_{\rho} g \bigr)^2 \\
%  & = \frac{1}{K} \Bigl( \var_{\rho} g + \bigl( \EE_{\wt{\rho}} g^2 - \EE_{\rho} g^2 \bigr) - \bigl( (\EE_{\wt{\rho}} g)^2 - (\EE_{\rho} g)^2 \bigr)\Bigr) + \bigl( \EE_{\wt{\rho}} g - \EE_{\rho} g \bigr)^2
%  \end{aligned}
%\end{equation*}
%Now consider a function $h$, choose $\Gamma$ to be the coupling between $\wt{\rho}$ and $\rho$ that minimizes the Wasserstein-$2$ metric, we have 
%\begin{equation*}
%  \begin{aligned}
%    \Abs{ \EE_{\wt{\rho}} h  - \EE_{\rho} h }  &= \Abs{ \int_{\RR^d \times \RR^d} \bigl(h(y) - h(z) \bigr)\, \Gamma(\ud y, \ud z) }  \\
%    & \leq  \int_{\RR^d \times \RR^d} \abs{y - z}\, \max\bigl\{ \abs{\nabla h(y)}, \abs{\nabla h(z)} \bigr\}\, \Gamma(\ud y, \ud z)  \\
%    & \leq \max\Bigl\{ \EE_{\wt{\rho}} \abs{\nabla h}^2, \EE_{\rho} \abs{\nabla h}^2  \Bigr\}^{1/2}  \biggl( \int_{\RR^d \times \RR^d} \abs{y - z}^2  \Gamma(\ud y, \ud z)\biggr)^{1/2} \\
%    & = \max\Bigl\{ \EE_{\wt{\rho}} \abs{\nabla h}^2, \EE_{\rho} \abs{\nabla h}^2  \Bigr\}^{1/2} W_2(\wt{\rho}, \rho). 
%    \end{aligned}
%\end{equation*}
%The lemma follows by applying the above to $h = g$ and $g^2$.
%\end{proof}
%
%
%To control the right hand side of \eqref{eq:msebound}, notice that
%$\nabla g(x) = a x e^{a\abs{x}^2/2}$ and
%$(g \nabla g) (x) = ax e^{a \abs{x}^2}$, thus
%\begin{equation}
%  \Abs{ g \nabla g(x)}^2 = a^2 \abs{x}^2 e^{2 a \abs{x}^2} \leq e^{(2a + a^2) \abs{x}^2} 
%\end{equation}
%Thus, for $a$ sufficiently
%small that $ \frac{1}{2a + a^2} \geq d \max \bigl\{ \norm{\wt{\rho}}_{\psi_2}^2
%,  \norm{\rho}_{\psi_2}^2\bigr\}$ (with
%slight abuse of notation, we denote
%$\norm{\rho}_{\psi_2} := \norm{X}_{\psi_2}$ for $X \sim \rho$), we
%have
%\begin{equation}
%  \max \Bigl\{ \EE_{\wt{\rho}} \abs{ g \nabla g }^2, \EE_{\rho} \abs{ g\nabla g }^2  \Bigr\} \leq 2.
%\end{equation}
%
%
%
%The Wasserstein-2 distance between $\rho$ and $\rho^{(n)}$ follows
%from the previous work \cite{DalalyanRiou-Durand}. 
%
%Consider discretized underdamped Langevin diffusion (with $\psi_0(t) = e^{-\gamma t}$ and $\psi_{j+1}(t) = \int_0^t \psi_j(s) \ud s$; note that $\psi_0(h) = \Or(1)$, and $\psi_{j}(h) = \Or(h^j)$)
%\begin{equation}
%  \begin{pmatrix}
%    v_{k+1} \\
%    x_{k+1} 
%  \end{pmatrix}
%  =
%  \begin{pmatrix}
%    \psi_0(h) v_k - \psi_1(h) \nabla f(x_k) \\
%    x_k + \psi_1(h) v_k - \psi_2(h) \nabla f(x_k) 
%  \end{pmatrix}
%  + \sqrt{2\gamma}
%  \begin{pmatrix}
%    \xi_k \\
%    \xi_k'
%  \end{pmatrix}
%\end{equation}
%with $(\xi_k, \xi_k')$ iid each component with covariance matrix
%\begin{equation*}
%  C_h := \int_0^h
%  \begin{pmatrix}
%    \psi_0(t) \\
%    \psi_1(t)
%  \end{pmatrix}
%  \begin{pmatrix}
%    \psi_0(t) & \psi_1(t)
%  \end{pmatrix} \ud t
%\end{equation*}
%The scheme solves in time interval $[kh, (k+1)h)$ the SDE
%\begin{equation}\label{eq:Langevin}
%  \ud
%  \begin{pmatrix}
%    V_t \\
%    X_t 
%  \end{pmatrix}
%  = \begin{pmatrix}
%    - \gamma V_t - \nabla f(X_{kh}) \\
%    V_t
%  \end{pmatrix} \ud t
%  + \sqrt{2\gamma}
%  \begin{pmatrix}
%    \ud W_t \\
%    0
%  \end{pmatrix}
%\end{equation}
%Denote $\rho_n$ the empirical distribution of $x_n$.  It is proved in
%\cite{DalalyanRiou-Durand} that for every $\gamma \geq \sqrt{\mu + L}$
%and $h \leq \mu / (4 \gamma L)$, it holds
%\begin{equation}
%  W_2(\rho_n, \rho) \leq \sqrt{2} \Bigl( 1 - \frac{3\mu h}{4 \gamma} \Bigr)^n W_2(\rho_0, \rho) + \frac{L h \sqrt{2d}}{\mu}, 
%\end{equation}
%which suggests the parameter choice 
%\begin{equation}
%  \gamma = \sqrt{\mu + L} \qquad \text{and} \qquad h = \min \biggl\{\frac{\mu}{4 L \sqrt{\mu + L}}, \frac{0.94 \veps}{\kappa \sqrt{2d}} \biggr\}, 
%\end{equation}
%which give the estimate of number of steps
%\begin{equation}
%  \begin{aligned}
%    n & \geq \frac{4 \sqrt{\mu + L}}{3 \mu} \frac{1}{h} \log \Bigl( \frac{24
%      W_2(\rho_0, \rho)}{\veps} \Bigr)  \\
%    & = 3 \kappa^{3/2} \biggl(\max\Bigl\{ 16 \kappa, \frac{d}{\mu
%      \veps^2} \Bigr\}\biggr)^{1/2} \log \Bigl( \frac{24
%      W_2(\rho_0, \rho)}{\veps} \Bigr) 
%  \end{aligned}
%\end{equation}
%to guarantee that $W_2(\rho_n, \rho) \leq \veps$. 
%
%
%Back to sub-Gaussianity, we consider the Orlicz norm of the random
%variable $Z$ 
%\begin{equation}
%  \norm{Z}_{\psi_2} := \inf\, \bigl\{ m \in (0, \infty) \mid \EE e^{(Z/m)^2} - 1 \leq 1 \bigr\}
%\end{equation}
%Thus for $\forall m \geq \norm{Z}_{\psi_2}$, 
%\begin{equation}
%  \EE e^{(Z / m)^2} \leq \EE e^{(Z / \norm{Z}_{\psi_2})^2} \leq 2. 
%\end{equation}
%The Orlicz $\psi_2$ norm is extended to multi-variate random variables
%$X \in \RR^d$ as
%\begin{equation}
%  \norm{X}_{\psi_2} = \sup_{\theta \in \mathbb{S}^{d-1}} \norm{ \average{\theta, X}}_{\psi_2}
%\end{equation}
%For any $ m \geq \norm{X}_{\psi_2}$, we again have 
%\begin{equation}
%  \EE\, e^{\frac{\abs{X}^2}{d m^2}} = \EE\, \exp\Bigl( \frac{1}{d} \sum_{i=1}^d \frac{X_i^2}{m^2} \Bigr) \stackrel{\text{(i)}}{\leq} \frac{1}{d} \sum_{i=1}^d \EE\, e^{X_i^2 / m^2} \stackrel{\text{(ii)}}{\leq} 2. 
%\end{equation}
%where (i) follows from Jensen's inequality and (ii) follows from that
%each component $X_i$ is sub-Gaussian with Orlicz norm
%$\norm{X}_{\psi_2}$ from the definition. 
%
%
%
%
%
%The SDE \eqref{eq:Langevin} has solution for $t \geq jh$
%\begin{align}
%  V_t & = e^{-\gamma (t - jh)}  V_{jh} - \int_{jh}^t e^{-\gamma(t - s)} \nabla f(X_s) \ud s + \sqrt{2\gamma} \int_{jh}^t e^{-\gamma(t - s)} \ud W_s \\
%  X_t & = X_{jh} + \int_{jh}^t V_s \ud s 
%\end{align}
%Consider another process $(V_t', X_t')$ with $(V_{jh}', X_{jh}') = (V_{jh}, X_{jh})$ and synchronous coupling (using the same $W_s$), we have
%\begin{align}
%  V_t' - V_t & =  e^{-\gamma(t - jh)} (V_{jh}' - V_{jh}) - \int_{jh}^t e^{-\gamma(t-s)}
%               \bigl( \nabla f(X_s') - \nabla f(X_s)\bigr)\ud s \\
%  X_t' - X_t & = (X_{jh}' - X_{jh}) + \int_{jh}^t (V_s' - V_s) \ud s 
%\end{align}
%
%\begin{equation}
%  \begin{aligned}
%    V_t' - V_t & =  e^{-\gamma(t - jh)} (V_{jh}' - V_{jh}) - \int_{jh}^t e^{-\gamma(t-s)} H_s (X_s' - X_s) \ud s \\
%    & = e^{-\gamma(t - jh)} (V_{jh}' - V_{jh}) - \int_{jh}^t
%    e^{-\gamma(t-s)} H_s \ud s \, (X_{jh}' - X_{jh}) - \int_{jh}^t
%    e^{-\gamma(t-s)} H_s \int_{jh}^s (V_u' - V_u) \ud u \ud s \\
%    & = e^{-\gamma(t - jh)} (V_{jh}' - V_{jh}) - \int_{jh}^t
%    e^{-\gamma(t-s)} H_s \ud s\, (X_{jh}' - X_{jh}) - \int_{jh}^t
%    \int_u^t e^{-\gamma(t-s)} H_s\ud s \, (V_u' - V_u)   \ud u \\
%  \end{aligned}
%\end{equation}
%
%\jl{Euclidean contraction leads to Orlicz norm contraction}
%
%% Recall from \cite{DalalyanRiou-Durand}*{Proposition 1} we have for
%% $\gamma \geq \sqrt{2 (L + \mu)}$
%% \begin{equation}
%%   \Abs{X_t - X_t'} \leq \Bigl( \frac{2\gamma^2 - 4 \mu}{\gamma^2 - 4 \mu} \Bigr)^{1/2} e^{- \mu t / \gamma} \Abs{X_0 - X_0'}
%% \end{equation}
%% Thus 
%% \begin{equation}
%%   \Norm{X_t - X_t'}_{\psi_2} \leq \Bigl( \frac{2\gamma^2 - 4 \mu}{\gamma^2 - 4 \mu} \Bigr)^{1/2} e^{- \mu t / \gamma} \Norm{X_0 - X_0'}_{\psi_2} 
%% \end{equation}
%Recall that we have (from the proof of \cite{DalalyanRiou-Durand}*{Proposition 1}) that for $\gamma \geq \sqrt{L + m}$
%\begin{equation}
%  \begin{pmatrix} 
%    \Abs{(V_t - V_t') + \gamma (X_t - X_t')} \\
%    \Abs{V_t - V_t'}
%  \end{pmatrix}
%  \leq e^{- \mu t / \gamma}
%  \begin{pmatrix} 
%    \Abs{(V_0 - V_0') + \gamma (X_0 - X_0')} \\
%    \Abs{V_0 - V_0'}
%  \end{pmatrix}, 
%\end{equation}
%which yields 
%\begin{equation}\label{eq:ContContract}
%  \begin{Vmatrix} 
%    (V_t - V_t') + \gamma (X_t - X_t') \\
%    V_t - V_t'
%  \end{Vmatrix}_{\psi_2} 
%  \leq e^{- \mu t / \gamma}
%  \begin{Vmatrix} 
%    (V_0 - V_0') + \gamma (X_0 - X_0') \\
%    V_0 - V_0'
%  \end{Vmatrix}_{\psi_2}. 
%\end{equation}
%We will use below this contraction of Orlicz norm for the SDE. 
%
%
%
%
%Now consider the sampling scheme written in integral form:
%\begin{align}
%  \wt{V}_t & = e^{-\gamma (t - jh)}  \wt{V}_{jh} - \int_{jh}^t e^{-\gamma(t - s)}  \ud s
%             \, \nabla f(\wt{X}_{jh}) + \sqrt{2\gamma} \int_{jh}^t e^{-\gamma(t - s)} \ud W_s \\
%  \wt{X}_t & = \wt{X}_{jh} + \int_{jh}^t \wt{V}_s \ud s 
%\end{align}
%To control the sub-Gaussianity, we subtract $(\wt{V}_t, \wt{X}_t)$ with a realization of the continuous underdamped Langevin process with initial distribution given by the invariant measure. 
%
%
%\begin{prop}
%  The random variable $\wt{X}_{kh}$ given by the underdamped Langevin sampling scheme at step $k$ is sub-Gaussian and
%  \begin{equation}
%    \norm{\wt{X}_{kh}}_{\psi_2} \leq \sqrt{2} h \kappa  + \biggl(1 + \sqrt{2} \Bigl( 1 - \frac{3\mu h}{4\gamma} \Bigr)^k \biggr) \norm{\rho}_{\psi_2}.
%  \end{equation}
%\end{prop}
%\begin{proof}
%Define matrix $P$ as 
%\begin{equation*}
%  P = \frac{1}{\gamma} 
%  \begin{pmatrix} 
%    0_{d\times d} & - \gamma I_{d\times d} \\
%    I_{d\times d} & I_{d\times d}
%  \end{pmatrix}, 
%  \quad 
%  \text{and} 
%  \quad 
%  P^{-1} = \begin{pmatrix} 
%    I_{d\times d} & \gamma I_{d\times d} \\
%    -I_{d\times d} & 0_{d\times d} 
%  \end{pmatrix}
%\end{equation*}
%Consider $(V_t, X_t)$ following the underdamped Langevin process with same noise and $(V_0, X_0)$ satisfying the equilibrium distribution. We would like to bound
%\begin{equation*}
%  A_k := \Norm{P^{-1} 
%    \begin{pmatrix} 
%      \wt{V}_{kh} - V_{kh} \\
%      \wt{X}_{kh} - X_{kh}
%    \end{pmatrix}}_{\psi_2} 
%\end{equation*}
%by introducing the auxiliary process $(V_t', X_t')$ such that
%$(V_{kh}', X_{kh}') = (\wt{V}_{kh}', \wt{X}_{kh}')$ and $(V_t', X_t')$
%satisfies the SDE \eqref{eq:Langevin} for $t \in [kh, (k+1)h)$. By
%triangular inequality
%\begin{equation}\label{eq:Ak1iter}
%  \begin{aligned}
%    A_{k+1} & \leq \Norm{P^{-1}
%      \begin{pmatrix} 
%        \wt{V}_{(k+1)h} - V_{(k+1)h}' \\
%        \wt{X}_{(k+1)h} - X_{(k+1)h}'
%      \end{pmatrix}}_{\psi_2} 
%    +  \Norm{P^{-1}     
%      \begin{pmatrix} 
%        V_{(k+1)h}' - V_{(k+1)h} \\
%        X_{(k+1)h}' - X_{(k+1)h}
%      \end{pmatrix}}_{\psi_2}  \\
%    & \stackrel{\eqref{eq:ContContract}}{\leq} \Norm{P^{-1}
%      \begin{pmatrix} 
%        \wt{V}_{(k+1)h} - V_{(k+1)h}' \\
%        \wt{X}_{(k+1)h} - X_{(k+1)h}'
%      \end{pmatrix}}_{\psi_2}  + e^{- \mu h / \gamma} A_k. 
%  \end{aligned}
%\end{equation}
%To control the first term on the right hand side, note that 
%\begin{equation*}
%  \begin{aligned}
%    \Norm{\wt{V}_t - V_t'}_{\psi_2} & = \Norm{ \int_{kh}^t e^{-\gamma(t-s)} \bigl(\nabla f(X_s') - \nabla f(X_{kh}') \bigr) \ud s  }_{\psi_2} \\
%    & \leq \int_{kh}^t \Norm{\nabla f(X_s') - \nabla f(X_{kh}')}_{\psi_2} \ud s \\
%    & \leq L \int_{kh}^t \Norm{ X_s' - X_{kh}' }_{\psi_2} \ud s \\
%    & \leq L \int_{kh}^t \int_{kh}^s \Norm{ V_u' }_{\psi_2} \ud u \ud s \\
%    & = L \int_{kh}^t (t - u) \Norm{ V_u' }_{\psi_2} \ud u \\
%    & \leq L \int_{kh}^t (t - u) \ud u \max_{u \in [kh, (k+1)h)} \Norm{ V_u' }_{\psi_2} \\
%    & = \frac{L(t - kh)^2}{2} \max_{u \in [kh, (k+1)h)} \Norm{ V_u' }_{\psi_2}.
%  \end{aligned}
%\end{equation*}
%In particular 
%\begin{equation*}
%  \Norm{\wt{V}_{(k+1)h} - V_{(k+1)h}'}_{\psi_2} \leq  \frac{L h^2}{2} \max_{u \in [kh, (k+1)h)} \Norm{ V_u' }_{\psi_2},
%\end{equation*}
%and moreover
%\begin{equation*}
%  \begin{aligned}
%    \Norm{\wt{X}_{(k+1)h} - X_{(k+1)h}'}_{\psi_2} & = \Norm{ \int_{kh}^{(k+1)h} 
%      (\wt{V}_t - V_t') \ud t }_{\psi_2}\\
%    & \leq \int_{kh}^{(k+1)h}  \Norm{\wt{V}_t - V_t'}_{\psi_2} \ud t \\
%    & \leq \frac{L}{2} \int_{kh}^{(k+1)h} (t - kh)^2 \ud t \max_{u \in [kh, (k+1)h)} \Norm{ V_u' }_{\psi_2} \\ 
%    & \leq \frac{Lh^3}{6} \max_{u \in [kh, (k+1)h)} \Norm{ V_u' }_{\psi_2}.
%  \end{aligned}
%\end{equation*}
%To control $\max_{u \in [kh, (k+1)h)} \Norm{ V_u' }_{\psi_2}$, we have
%\begin{equation*}
%  \begin{aligned}
%    \Norm{ V_u' }_{\psi_2} & \leq \Norm{ V_u }_{\psi_2} + \Norm{ V_u' - V_u }_{\psi_2} \\
%    & = 1 + \Norm{ 
%      \begin{pmatrix} 
%        I_{d\times d} & 0_{d\times d}
%      \end{pmatrix} 
%      P P^{-1} 
%      \begin{pmatrix}
%        V_u' - V_u \\
%        X_u' - X_u 
%      \end{pmatrix}
%    }_{\psi_2} \\
%    & \leq 1 + \Abs{\begin{pmatrix}
%        I_{d\times d} & 0_{d\times d}
%      \end{pmatrix} 
%      P} \Norm{P^{-1} 
%      \begin{pmatrix}
%        V_u' - V_u \\
%        X_u' - X_u 
%      \end{pmatrix}
%    }_{\psi_2} \\
%    & \leq 1 + \Norm{P^{-1} 
%      \begin{pmatrix}
%        V_{kh}' - V_{kh} \\
%        X_{kh}' - X_{kh} 
%      \end{pmatrix}
%    }_{\psi_2} \\
%    & = 1 + A_k. 
%  \end{aligned}
%\end{equation*}
%Thus 
%\begin{equation*}
%  \Norm{P^{-1}
%    \begin{pmatrix} 
%      \wt{V}_{(k+1)h} - V_{(k+1)h}' \\
%      \wt{X}_{(k+1)h} - X_{(k+1)h}'
%    \end{pmatrix}}_{\psi_2} \leq \biggl( \bigl( 1 + \frac{\gamma
%    h}{3}\bigr)^2 + 1 \biggr)^{1/2} \frac{Lh^2}{2} ( 1 + A_k ) \leq
%  0.75 L h^2 ( 1 + A_k)
%\end{equation*}
%by choosing $h \leq 1 / (4 \gamma)$. Combined with \eqref{eq:Ak1iter},
%we arrive at
%\begin{equation*}
%  A_{k+1} \leq 0.75 L h^2 ( 1 + A_k) + e^{-h\mu / \gamma} A_k.
%\end{equation*}
%The iteration gives 
%\begin{equation*}
%  A_k \leq \frac{L h \gamma}{\mu} + \Bigl( 1 - \frac{3\mu h}{4\gamma} \Bigr)^k A_0 
%\end{equation*}
%Thus, 
%\begin{equation*}
%  \begin{aligned}
%  \norm{\wt{X}_{kh} - X_{kh}}_{\psi_2} & \leq \Abs{\begin{pmatrix}
%      0_{d\times d} & I_{d\times d} 
%      \end{pmatrix} 
%      P} A_k = \gamma^{-1} \sqrt{2} A_k \\
%    & \leq \frac{Lh\sqrt{2}}{\mu} + \gamma^{-1} \sqrt{2} \Bigl( 1 - \frac{3\mu h}{4\gamma} \Bigr)^k A_0 \\
%    & = \frac{Lh\sqrt{2}}{\mu} + \sqrt{2} \Bigl( 1 - \frac{3\mu h}{4\gamma} \Bigr)^k \norm{\wt{X}_0 - X_0}_{\psi_2} \\
%    &  = \frac{Lh\sqrt{2}}{\mu} + \sqrt{2} \Bigl( 1 - \frac{3\mu h}{4\gamma} \Bigr)^k \norm{\rho}_{\psi_2}.
%  \end{aligned}
%\end{equation*}
%Since $X_{kh} \sim \rho$ by construction, we get 
%\begin{equation*}
%  \norm{\wt{X}_{kh}}_{\psi_2} \leq \sqrt{2} h \kappa  + \biggl(1 + \sqrt{2} \Bigl( 1 - \frac{3\mu h}{4\gamma} \Bigr)^k \biggr) \norm{\rho}_{\psi_2}, 
%\end{equation*}
%which is the conclusion of the proposition.
%\end{proof}
%
%Recall the choice of $\gamma = \sqrt{\mu + L}$ and $h = \min \biggl\{\frac{\mu}{4 L \sqrt{\mu + L}}, \frac{0.94 \veps}{\kappa \sqrt{2d}} \biggr\}$, we arrive at \jlnotes{check the constant $2$}
%\begin{equation}
%  \norm{\wt{X}_{kh}}_{\psi_2} \leq \min \biggl\{\frac{\sqrt{2}}{4\sqrt{\mu + L}}, \frac{0.94 \sqrt{2} \veps}{\sqrt{2d}} \biggr\} + 2 \norm{\rho}_{\psi_2}. 
%\end{equation}
%
%Hence, this in turn requires the parameters in \eqref{eq:gdef} satisfying (we have dropped the term with $\veps$ dependence) \jlnotes{switched back to the $\mu$ and $L$ for the given $\rho$ here} 
%\begin{equation}
%  \begin{aligned}
%    \frac{\sigma^2}{\alpha} & \geq d \biggl( \frac{\sqrt{2}}{4\sqrt{\mu + L + \sigma^{-2}}} + 2 \norm{\rho}_{\psi_2}\biggr)^2 \\
%    & = d \biggl( \frac{\sqrt{2}}{4\sqrt{\mu + L + \sigma^{-2}}} +  \frac{2}{\sqrt{\mu + \sigma^{-2}}}\biggr)^2
%  \end{aligned}
%\end{equation}
%which is satisfied as long as $\alpha \leq \max\{\frac{1}{3d}, \frac{\mu \sigma^2}{d}\}$.
%
%
%\bibliographystyle{amsxport}
%\bibliography{sampling}
%
%
%
%\end{document}
%
%
%% using Ito's lemma,
%% \begin{equation}
%%   \ud e^{a\abs{X_t}^2} = 2a V_t \cdot X_t e^{a\abs{X_t}^2} \ud t
%% \end{equation}
%% More directly, using the solution of the SDE
%% \begin{align}
%%   \exp\bigl(a \abs{x_{k+1}}^2\bigr) & =
%%   \exp\Bigl(a \Abs{x_k + \psi_1(h) v_k - \psi_2(h) \nabla f(x_k) +
%%     \sqrt{2\gamma} \xi_k'}^2\Bigr)\\
%%   \exp\bigl(a \abs{v_{k+1}}^2\bigr) & =
%%   \exp\Bigl(a \Abs{\psi_0(h) v_k - \psi_1(h) \nabla f(x_k) + \sqrt{2\gamma} \xi_k}^2  \Bigr)
%% \end{align}
%% Thus
%% \begin{equation}
%%   \begin{aligned}
%%     \EE \exp\bigl(a \abs{x_{k+1}}^2\bigr) & = \EE \exp\Bigl(a \Abs{x_k
%%       + \psi_1(h) v_k - \psi_2(h) \nabla f(x_k) +
%%       \sqrt{2\gamma} \xi_k'}^2\Bigr)\\
%%         & = \EE \exp\Bigl(a \Abs{x_k + \psi_1(h) v_k - \psi_2(h) \nabla
%%       f(x_k) }^2\Bigr) \exp\Bigl( 2 a \sqrt{2\gamma}
%%     \bigl(x_k + \psi_1(h) v_k - \psi_2(h) \nabla
%%     f(x_k)\bigr) \cdot \xi_k' + 2 a \gamma \abs{\xi_k'}^2 \Bigr) \\
%%     & = \biggl(\frac{2\pi}{\frac{1}{\var \xi_k'} - 4a\gamma} \biggr)^{d/2} \EE \exp\Bigl( \frac{a}{1 - 4 a \gamma \var \xi_k'}  \Abs{x_k + \psi_1(h) v_k - \psi_2(h) \nabla
%%       f(x_k) }^2 \Bigr)
%%   \end{aligned}
%% \end{equation}
%
%% \begin{equation}
%%   \begin{aligned}
%%     \EE \exp\bigl(a \abs{v_{k+1}}^2\bigr) & = \EE \exp\Bigl(a
%%     \Abs{\psi_0(h) v_k - \psi_1(h) \nabla f(x_k) + \sqrt{2\gamma}
%%       \xi_k }^2 \Bigr) \\
%%     & = \EE \exp\Bigl(a \Abs{\psi_0(h) v_k - \psi_1(h) \nabla
%%       f(x_k)}^2\Bigr)
%%     \exp\Bigl(2a\sqrt{2\gamma} \bigl( \psi_0(h) v_k - \psi_1(h) \nabla f(x_k)\bigr) \cdot \xi_k + 2a\gamma \abs{\xi_k}^2 \Bigr) \\
%%     & = \biggl(\frac{2\pi}{\frac{1}{\var \xi_k} - 4a\gamma}
%%     \biggr)^{d/2} \EE \exp\Bigl( \frac{a}{1 - 4 a \gamma \var \xi_k}
%%     \Abs{\psi_0(h) v_k - \psi_1(h) \nabla f(x_k)}^2 \Bigr) \\
%%     & \leq \biggl(\frac{2\pi}{\frac{1}{\var \xi_k} - 4a\gamma}
%%     \biggr)^{d/2} \EE \exp\Bigl( \frac{2 a \psi_0(h)^2}{1 - 4 a \gamma
%%       \var \xi_k} \abs{v_k}^2\Bigr) \exp\Bigl( \frac{2 a \psi_1(h)^2}{1 - 4 a \gamma
%%       \var \xi_k} (L \abs{x_k})^2\Bigr) 
%%   \end{aligned}
%% \end{equation}
%% \jl{need to be careful that $x_k$ and $v_k$ are not independent; can we use Cauchy-Schwarz and sacrifice a factor of $2$? otherwise, need to track the  moments of the joint distribution}
%
%
%
%% Using the Laplace transform condition for sub-Gaussianity: 
%% \begin{equation}
%%   \begin{aligned}
%%     \EE e^{a \abs{x_k} + b \abs{v_k}} \lesssim e^{c (a^2 + b^2)}
%%   \end{aligned}
%% \end{equation} 
%
%% \begin{equation}
%%   \begin{aligned}
%%   \EE e^{a \abs{x_{k+1}} + b \abs{v_{k+1}}} & = \EE \exp \biggl( a \Abs{ x_k + \psi_1(h) v_k - \psi_2(h) \nabla f(x_k) + \sqrt{2\gamma} \xi_k'}  \\
%%   & \qquad \qquad + b \Abs{ \psi_0(h) v_k - \psi_1(h) \nabla f(x_k) + \sqrt{2 \gamma} \xi_k }  \biggr) \\ 
%%   & \leq \EE \exp \biggl( a \abs{x_k}  +  (b \psi_1(h) + a\psi_2(h)) \abs{\nabla f(x_k)} + (b \psi_0(h) + a \psi_1(h)) \abs{v_k}  \biggr)  \exp \Bigl(a \sqrt{2\gamma} \abs{ \xi_k' } + b \sqrt{2\gamma}\abs{ \xi_k }\Bigr) \\
%%   & \leq M_{a, b} \EE \exp \biggl( (a + b \psi_1(h) L + a \psi_2(h) L) \abs{x_k} 
%%   + (b \psi_0(h) + a \psi_1(h)) \abs{v_k} \biggr), 
%% \end{aligned}
%% \end{equation}
%% where 
%% \begin{equation}
%%   M_{a, b} = \EE e^{\sqrt{2\gamma} ( a \abs{\xi_k'} + b \abs{\xi_k})} 
%% \end{equation}
%
%% in the scheme
%% \begin{equation}
%%   \begin{aligned}
%%     \norm{v_{k+1}}_{\psi_2} & \leq \psi_0(h) \norm{v_k}_{\psi_2} + \psi_1(h) \norm{\nabla f(x_k)}_{\psi_2} + \sqrt{2\gamma} \norm{\xi_k}_{\psi_2}  \\
%%     & \leq \psi_0(h) \norm{v_k}_{\psi_2} + \psi_1(h) L \norm{x_k}_{\psi_2} + \sqrt{2\gamma} \norm{\xi_k}_{\psi_2}
%%   \end{aligned}
%% \end{equation}
%% Similarly 
%% \begin{equation}
%%   \begin{aligned}
%%     \norm{x_{k+1}}_{\psi_2} & \leq \norm{x_k - \psi_2(h) \nabla
%%       f(x_k)}_{\psi_2} + \psi_1(h)
%%     \norm{v_k}_{\psi_2} + \sqrt{2\gamma} \norm{\xi_k'}_{\psi_2} \\
%%     & \leq (1 - \psi_2(h) \mu) \norm{x_k}_{\psi_2} + \psi_1(h)
%%     \norm{v_k}_{\psi_2} + \sqrt{2\gamma} \norm{\xi_k'}_{\psi_2}
%% \end{aligned}
%% \end{equation}
%
%% Thus 
%% \begin{equation}
%%   \begin{pmatrix} 
%%     \norm{v_{k+1}}_{\psi_2} \\
%%     \norm{x_{k+1}}_{\psi_2}
%%   \end{pmatrix} 
%%   \leq 
%%   \begin{pmatrix} 
%%     \psi_0(h) & \psi_1(h) L \\
%%     \psi_1(h) & 1 - \psi_2(h) \mu
%%   \end{pmatrix}
%%   \begin{pmatrix} 
%%     \norm{v_{k}}_{\psi_2} \\
%%     \norm{x_{k}}_{\psi_2}
%%   \end{pmatrix} 
%%   + \sqrt{2\gamma} 
%%   \begin{pmatrix} 
%%     \norm{\xi_{k}}_{\psi_2} \\
%%     \norm{\xi_{k}'}_{\psi_2}
%%   \end{pmatrix} 
%% \end{equation}
%
%% \begin{equation}
%%   \Abs{\begin{pmatrix} 
%%     \psi_0(h) & \psi_1(h) L \\
%%     \psi_1(h) & 1 - \psi_2(h) \mu 
%%   \end{pmatrix}} \leq 1 + c h \max(\gamma, L)
%% \end{equation}
%
%% \begin{equation}
%%   \norm{x_k}_{\psi_2} \leq \bigl(1 + c h \max(\gamma, L) \bigr)^k \norm{v_0}_{\psi_2} + c k h \sqrt{2\gamma} \bigl(1 + c h \max(\gamma, L) \bigr)^k 
%% \end{equation}
%
%
%
%% \begin{proof}
%% \jl{the below is not enough; have to rely on a similar proof as Cousin-Vempala?}
%% \begin{equation}
%%   \begin{aligned}
%%     \frac{1}{2} \Bigl( - f(x) - \frac{1+\alpha}{2}
%%     \frac{\abs{x}^2}{\sigma^2} \Bigr) & + \frac{1}{2} \Bigl( - f(y) -
%%     \frac{1-\alpha}{2}
%%     \frac{\abs{y}^2}{\sigma^2} \Bigr) \\
%%     & = - \frac{1}{2} \bigl(f(x) + f(y)\bigr) -
%%     \frac{\abs{x}^2 + \abs{y}^2 }{4\sigma^2} + \frac{\alpha}{4\sigma^2} \bigl( \abs{y}^2 - \abs{x}^2 \bigr)  \\
%%     & \leq - f\Bigl( \frac{x+y}{2} \Bigr) - \frac{\mu}{4} \abs{x- y}^2
%%     - \frac{1}{2\sigma^2} \Abs{\frac{x+y}{2}}^2 - \frac{1}{2\sigma^2}
%%     \Abs{\frac{x-y}{2}}^2 +
%%     \frac{\alpha}{4\sigma^2}  (y - x) \cdot (y + x)  \\
%%     & \leq - f\Bigl( \frac{x+y}{2} \Bigr) - \frac{1}{2\sigma^2}
%%     \Abs{\frac{x+y}{2}}^2
%%     - \frac{1}{8\sigma^2}\Bigl( (y - x) - \alpha (y + x) \Bigr)^2 + \frac{\alpha^2}{2\sigma^2}  \Abs{\frac{x + y}{2}}^2 \\
%%     & \leq - f\Bigl( \frac{x+y}{2} \Bigr) - \frac{1}{2\sigma^2}
%%     \Abs{\frac{x+y}{2}}^2 + \frac{\alpha^2}{2\sigma^2} \Abs{\frac{x +
%%         y}{2}}^2
%% \end{aligned}
%% \end{equation} 
%% Thus by Prekopa-Leindler inequality, 
%% \begin{equation} 
%%   \begin{aligned}
%%     \int e^{- f(x) - \frac{1+\alpha}{2} \frac{\abs{x}^2}{\sigma^2}} \ud x \int
%%     e^{- f(x) -  \frac{1-\alpha}{2} \frac{\abs{x}^2}{\sigma^2}}  \ud x \leq \Biggl( \int e^{-f(x) - \frac{1-\alpha^2}{2}   \frac{\abs{x}^2}{\sigma^2}} \ud x 
%% \Biggr)^2. 
%%   \end{aligned}
%% \end{equation}
%% Therefore 
%% \begin{equation}
%%   \begin{aligned}
%%   \frac{\EE_{\rho_i}(g_i^2)}{\EE_{\rho_i} (g_i)^2} & \leq 
%%   \dfrac{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{1-\alpha^2}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\biggr)^2}{\biggl(\EE_{\rho}  \exp\Bigl(-\frac{1}{2} \frac{\abs{x}^2}{\sigma^2}\Bigr)\biggr)^2} \\
%%   & = \biggl( \EE_{\rho_{i+1}} \exp\Bigl( \frac{\alpha^2}{2\sigma^2} \abs{x}^2 \Bigr) \biggr)^2 
%% \end{aligned}
%% \end{equation}
%% which is $\Or(1)$ if
%% $\frac{\alpha^2}{\sigma^2} = \Or(\frac{1}{d})$,\jlnotes{this can
%%   actually be further relaxed especially for $\sigma \ll 1$} which is
%% guaranteed by the choice
%% $\alpha = c \max\{\frac{1}{d}, \frac{\sigma}{\sqrt{d}}\}$
%
%% \jl{however, we not only needed to be $\Or(1)$, but $1 + \Or(\frac{1}{d})$; requires a sharper analysis}
%% \end{proof}
%
%Below is a slightly simplified proof of \cite{CousinsVempala:2018}*{Lemma 7.6}. 
%
%
%% \begin{lemma}[\cite{CousinsVempala:2018}*{Lemma 7.6}] Let $[\ell, u] \subset [-R, R]$ and
%%   $\alpha \leq \frac{1}{2}$. Then for any $\gamma > 0$, 
%%   \begin{equation}
%%     \dfrac{ \int_{\ell}^u \exp(\gamma t) \exp \Bigl(- \frac{t^2(1 + \alpha)}{2 \sigma^2} \Bigr) \ud t
%%       \int_{\ell}^u \exp(\gamma t) \exp\Bigl( - \frac{t^2 (1 - \alpha)}{2 \sigma^2}\Bigr) \ud t}
%%     { \biggl( \int_{\ell}^u \exp(\gamma t) \exp \Bigl( - \frac{t^2}{2\sigma^2} \Bigr) \ud t \biggr)^2}
%%     \leq \exp \Bigl(2 \alpha^2 R^2 \sigma^{-2} \Bigr)  
%%   \end{equation}
%  
%% \end{lemma}
%
%% \begin{proof}
%%   Define the short hand notations
%%   \begin{equation*}
%%     s(x, t) := \exp(\gamma t) \exp\Bigl( -\frac{t^2x}{2\sigma^2} \Bigr)
%%   \end{equation*}
%%   and
%%   \begin{equation*}
%%     h(\alpha) := \dfrac{\int_{\ell}^u s(1+\alpha, t) \ud t \int_{\ell}^u s(1 - \alpha, t) \ud t}{\biggl( \int_{\ell}^u s(1, t) \ud t \biggr)^2}. 
%%   \end{equation*}
%%   Since it is clear that $h(0) = 1$, similar to the proof of the previous lemma, it suffices to show that
%%   \begin{equation}
%%     h'(\alpha) \leq 4 \alpha h(\alpha) \frac{R^2}{\sigma^2}.
%%   \end{equation}
%%   Direct calculations yield that 
%%   \begin{equation*}
%%     \dfrac{h'(\alpha)}{h(\alpha)} = \frac{1}{2\sigma^2} \Biggl(
%%     \dfrac{\int_{\ell}^u t^2 \exp(\gamma t) \exp\Bigl(-\frac{t^2 (1 - \alpha)}{2 \sigma^2}\Bigr) \ud t}{\int_{\ell}^u \exp(\gamma t) \exp\Bigl(-\frac{t^2 (1 - \alpha)}{2 \sigma^2}\Bigr) \ud t}
%%     - \dfrac{\int_{\ell}^u t^2 \exp(\gamma t) \exp\Bigl(-\frac{t^2 (1 + \alpha)}{2 \sigma^2}\Bigr) \ud t}{\int_{\ell}^u \exp(\gamma t) \exp\Bigl(-\frac{t^2 (1 + \alpha)}{2 \sigma^2}\Bigr) \ud t}
%%     \Biggr)
%%   \end{equation*}
%%   Let
%%   \begin{equation*}
%%     v(y) = \dfrac{\int_{\ell}^u t^2 \exp(\gamma t) \exp\Bigl(-\frac{t^2 y}{2 \sigma^2}\Bigr) \ud t}{\int_{\ell}^u \exp(\gamma t) \exp\Bigl(-\frac{t^2 y }{2 \sigma^2}\Bigr) \ud t}, 
%%   \end{equation*}
%%   we have then
%%   \begin{equation*}
%%     \dfrac{h'(\alpha)}{h(\alpha)} = - \frac{1}{2\sigma^2} \int_{1-\alpha}^{1+\alpha} v'(y) \ud y
%%   \end{equation*}
%%   We calculate
%%   \begin{equation*}
%%     v'(y) = \frac{1}{2\sigma^2} \dfrac{\Biggl(\int_{\ell}^u t^2 s(y, t) \ud t\Biggr)^2 - \int_{\ell}^u s(y, t) \ud t \int_{\ell}^u t^4 s(y, t)\ud t}{\Biggl(\int_{\ell}^u s(y, t) \ud t\Biggr)^2}
%%   \end{equation*}
%%   Let $Y$ be a Gaussian random variable
%%   $Y \sim \mathcal{N}\bigl(\frac{\gamma\sigma^2}{y},
%%   \frac{\sigma^2}{y} \bigr) $, we can write the above as
%%   \begin{equation*}
%%     \begin{aligned}
%%       v'(y) & = \frac{1}{2\sigma^2} \bigl( \EE(Y^2 \mid Y \in [\ell, u])^2 - \EE(Y^4 \mid Y \in [\ell, u]) \bigr) \\
%%       & = - \frac{1}{2\sigma^2} \var(Y^2\mid Y \in [\ell, u]) 
%%     \end{aligned}
%%   \end{equation*}
%%   Employing the Gaussian Poincar\`e inequality (on truncated intervals) $\var f(Y) \leq 4 \sigma^2y^{-1} \EE \abs{f'(Y)}^2$, we have 
%%   \begin{equation*}   
%%     \begin{aligned}
%%     \var(Y^2\mid Y \in [\ell, u]) \leq 4 \frac{\sigma^2}{y} \EE( Y^2 \mid Y \in [\ell, u]) \leq     4\frac{\sigma^2}{y} R^2.
%%     \end{aligned}
%%   \end{equation*}
%%     Thus,
%%   \begin{equation*}
%%     \begin{aligned}
%%       \dfrac{h'(\alpha)}{h(\alpha)} & \leq \frac{1}{2\sigma^2}  \int_{1-\alpha}^{1+\alpha}
%%       2 R^2 y^{-1} \ud y \\
%%       & = \frac{R^2}{\sigma^2} \ln\Bigl(\frac{1+\alpha}{1-\alpha}\Bigr)
%%         \\
%%       & \leq 4 \alpha \frac{R^2}{\sigma^2}. 
%%     \end{aligned}\qedhere
%%   \end{equation*}
% 
%  
%% \end{proof}


==> recycle.tex <==
\section{Recycle}

\subsection{Coupled points stay close with high probability}
\label{ss:couple}

\hlcom{This section is mostly unnecessary for a constant-probability result.}
%{Lemma~\ref{l:doob} and~\ref{l:bounded-E} are not necessary for a constant-probability result.}
We need a high-probability bound on how large the velocity can get. This will follow from a high-probability bound on the energy of the continuous system.
\begin{lem}\label{l:doob}
Suppose that $\ud X_t = u_t \dB_t$, where $u_t$ is continuous, square-integrable, and adapted to the filtration of $\dB_t$. %predictable...
Then
\begin{align}
\Pj\pa{\sup_{0\le t\le T} X_t-X_0 \ge C} &\le \exp\pa{-\fc{C^2}{2\int_0^T u_t^2\,dt}}.
\end{align}•
\end{lem}
\begin{proof}
Let $\la>0$. 
Note that $\exp(\la X_t)$ is a positive submartingale. By Doob's martingale inequality,
\begin{align*}
&\Pj(\sup_{0\le t\le T} X_t \ge C)  \le 
\Pj\pa{\sup_{0\le t\le T} \exp(X_t) \ge \exp(C)}\\
&\le 
\E\pf{\exp(\la X_T)}{\exp(\la C)}=\exp\pa{\rc 2 \la^2 \int_0^T u_t^2 \dt -\la C}.
\end{align*}
Choosing $\la = \fc{C}{\int_0^T u_t^2\dt}$ gives the bound.
\end{proof}
\begin{lem}\label{l:bounded-E}
Suppose that $f$ is %$\mu$-convex,  %not nec?
$L$-smooth and has minimum value $f(0)=0$.
Define $E_t = f(x_t) + \rc{2u}\ve{v_t}^2$. 
Suppose $D\ge 2\pa{E_0+\ga dT}$.
Then
\begin{align*}
\Pj\pa{
\sup_{0\le t\le T} E_t > D
%E_0 + \Dval %2\ga dT + 16u \log \pf{2}{\ep}
}&\le %\ep.
2\exp\pa{-\fc{D}{32\ga T}}
\end{align*}
\end{lem}
\begin{proof}
By It\^o's Lemma,
\begin{align}
\ud\pa{\rc 2 \ve{v_t}^2}
&= (-\ga \ve{v_t}^2 - \an{v_t,u\nb f(x_t)} + \ga ud) \dt + \sqrt{2\ga u} \ve{v_t}\dB_t\\
\ud(f(x_t))&=\an{\nb f(x_t),v_t}\\
\implies
\ud E_t 
=\ud\pa{\rc{2u}\ve{v_t}^2 + f(x_t)}
&= \pa{-\fc{\ga}{u} \ve{v_t}^2 + \ga d}\dt + \sfc{2\ga}u \ve{v_t}\dB_t
%&\le \ga d \dt + \sqrt{2u E_t}\dB_t
\end{align}
Consider the stochastic processes $E'_t,E_t''$ defined by
\begin{align}
\ud E'_t &= \ga d\dt + \sfc{2\ga}u\ve{v_t}\dB_t,
& E'_0=E_0\\
\ud E''_t &= \ga d\dt + \pa{\sfc{2\ga}u\ve{v_t}\vee 2\sqrt{\ga D}}\dB_t,
& E''_0=E_0
\end{align}
We can couple the processes $E_t,E_t',E_t''$ so that $E_t\le E_t'$ and conditioned on $E_t\le D$ for $0\le t\le T$, we have $E_t'= E_t''$. This is since $\ve{v_t}\le\sqrt{2u E_t}$. Then by Lemma~\ref{l:doob} applied to the martingale $E_t'' - \ga dt$, 
\begin{align*}
\Pj\pa{\sup_{0\le t\le T} E''_t \ge D}
&\le \Pj\pa{\sup_{0\le t\le T} (E''_t-E_0-\ga dt)\ge D-E_0-\ga dT}\\
%&\le 2\exp\Pj(E_T'-\ga dT \ge E_0+D-\ga dT)\\
&\le 2\exp\pa{-\fc{(D-E_0-\ga dT)^2}{8\ga DT}}\\
&\le 2\exp\pa{-\fc{D}{32\ga T}}%&\text{using }D-\ga dT \ge \fc D2.
\end{align*}
where the last step uses $D-(E_0+\ga dT) \ge \fc D2$.
%Finally, note that $\sup_{0\le t\le T} E_t'' <D$ iff $\sup_{0\le t\le T} E_t <D$.
Now, if $\sup_{0\le t\le T} E_t'' <D$, then $\sup_{0\le t\le T} E_t< D$ and $E_t\le E_t''$. Thus 
$\Pj\pa{\sup_{0\le t\le T} E_t \ge E_0+D} \le 2\exp\pa{-\fc{D}{32\ga T}}$. 
\end{proof}

Let $F(x,v,y,w):= \ve{(x+v)-(y+w)}^2 + \ve{x-y}^2$. 
\begin{lem}\label{l:cont-couple}
Suppose that $(x_t,v_t)$ and $(y_t,w_t)$ are synchronously coupled continuous processes. Then 
\begin{align}
F(x_t,v_t,y_t,w_t) &\le e^{-\fc{t}{\ka}} F(x_0,v_0,y_0,w_0).
\end{align}•
\end{lem}
\begin{proof}
This follows from the proof of Theorem 5 in~\cite{cheng2017underdamped}. (Note that the expectations are taken only at the end.)
\end{proof}
\begin{lem}\label{l:cont-disc}
Suppose that $(x_s,v_s)$ and $(\wt x_s,\wt v_s)$ are synchronously coupled continuous and discrete processes with $x_0=\wt x_0$, $v_0=\wt v_0$, $s\le \eta$. Suppose that $\sup_{0\le r\le s}\ve{v_r}^2\le \cal E_K$. Let $\ga =2$. Then
\begin{align}
\ve{v_s-\wt v_s}_2^2&\le \fc{s^4u^2L^2\cal E_K}{3}\\
\ve{x_s-\wt x_s}_2^2&\le \fc{s^6u^2L^2\cal E_K}{15}\\
\ve{(x_s+v_s)-(\wt x_s+\wt v_s)}_2^2 + 
\ve{x_s-\wt x_s}_2^2 &\le s^4u^2L^2 \cal E_K\pa{\fc{s^2}5+\fc 23}.
\end{align}
\end{lem}
\begin{proof}
This follows from the calculation in Theorem 9 in~\cite{cheng2017underdamped}, but without the expectations. For the last part, note that 
\begin{align*}
\ve{(x_s+v_s)-(\wt x_s+\wt v_s)}_2^2 + 
\ve{x_s-\wt x_s}_2^2 
&\le 3\ve{x_s-\wt x_s}_2^2 + 2\ve{v_s-\wt v_s}_2^2.
\end{align*}
\end{proof}

\begin{lem}\label{l:cont-disc2}
Let $(\wt x_s,\wt v_s)$ be the discrete process with step size $\eta\le \rc{8\sqrt 2\ka}$. 
Suppose that $(x_s,v_s)$ and $(\wt x_s,\wt v_s)$ are synchronously coupled continuous and discrete processes with $x_0=\wt x_0$, $v_0=\wt v_0$. 
Suppose that $\sup_{0\le t\le T} E_t<\cal E$ and $\cal E\ge 2(E_0+\ga dT)$. Then for all $0\le t\le T$,
$$
\ve{(x_t+v_t)-(\wt x_t+\wt v_t)}_2^2 + 
\ve{x_t-\wt x_t}_2^2 \le 
\fc{128 \ka^2 \eta^2 \cal E}L.
$$
\end{lem}
Here $T$ will be on the order of 1 and $\cal E$ will be on the order of $d$, so we get that $x_T,\wt x_T$ will be at distance $\cO(\sqrt{d})$ with high probability.
\begin{proof}
%Let $F(x,v,y,w):= \ve{(x+v)-(y+w)}^2 + \ve{x-y}^2$. 
%By Lemma~\ref{l:bounded-E}, with probability $\ge1-\ep$ we have $\sup_{0\le t\le T} E_t \le \cal E$. 
%Under this event, 
We have $\ve{v_t}_2^2\le \fc{2E_t}L\le \fc{2\cal E}L$ for $0\le t\le T$.
Let $\cal E_K = \fc{8\cal E}L$.
%We show by induction on $t$ that 
We will show that for $0\le t\le T$,
\begin{align}
\label{e:induct1}
\sqrt{F(\wt x_t, \wt v_t, x_t,v_t)}&\le \sumz j{\ce{\fc{t}{\eta}}-1}e^{-\fc{\eta j}{2\ka}}\eta^2 \sqrt{\cal E_K}
\end{align}
%Note that the second inequality implies
%\begin{align}
%\ve{\wt v_t} &\le \sqrt{2u\cal E} + \ve{v_t} \fc{\sqrt 2}{1-e^{-\eta/(2\ka)}} \eta^2 \sqrt{\cal E_K}
%\le \sqrt{\cal E_K}.
%\end{align}

We now prove~\eqref{e:induct1} %and~\eqref{e:induct2} 
by induction: 
Suppose~\eqref{e:induct1} holds up to $t$; we show it holds up to $t+\eta$. 
For $s\ge t$, let $(y_s,w_s)$ be the continuous dynamics started at $(\wt x_t,\wt v_t)$. 
First we note that by Lemma~\ref{l:cont-couple},
\begin{align}
\label{e:Fyw}
\sqrt{F(y_{t+r}, w_{t+r}, x_{t+r},v_{t+r})}
&\le  e^{-\fc{r}{2\ka}} \sqrt{F(y_{t}=\wt x_t, w_{t}=\wt v_t, x_{t},v_{t})}.
\end{align}
and
\begin{align}
\label{e:Fxv}
 \sqrt{F(\wt x_t,\wt v_t, x_{t},v_{t})}
& \le \fc{1}{1-e^{-\eta/(2\ka)}} \eta^2 \sqrt{\cal E_K}
\le \fc{\eta^2}{\eta/(4\ka)} \sfc{8\cal E}{L}
\le \sqrt{\fc{\cal E}{L}}.
\end{align}
by the assumption $\eta\le \rc{8\sqrt 2\ka}$. 
%$\fc{\eta^2}{1-e^{-\fc{\eta}{2\ka}}}\le \rc{2\sqrt 2}$.
Then for $0\le r\le \eta$,
\begin{align}
\label{e:induct2}
\ve{w_{t+r}} &\le \ve{v_{t+r}} + \ve{w_{t+r}-v_{t+r}}\\
&\le \ve{v_{t+r}} + \sqrt{2} \sqrt{F(y_{t+r},w_{t+r},x_{t+r},v_{t+r})}\\
&\le   \sqrt{\fc{2\cal E}{L}}+\sqrt{\fc{2\cal E}{L}}=\sqrt{\cal E_K}
\end{align}
Hence we can apply Lemma~\ref{l:cont-disc} to $(y_s,w_s)$ and $(\wt x_s,\wt v_s)$. 
Then by Minkowski's inequality, for $0\le r\le \eta$,
\begin{align}
\sqrt{F(\wt x_{t+r}, \wt v_{t+r}, x_{t+r},v_{t+r})}
&\le 
\sqrt{F(y_{t+r}, w_{t+r}, x_{t+r},v_{t+r})}
+
\sqrt{F(\wt x_{t+r}, \wt v_{t+r}, y_{t+r},w_{t+r})}\\
%\ve{\wt v_{t+\eta} - v_{t+\eta}}_2
%&\le 
%\ve{w_{t+\eta}-v_{t+\eta}}_2 + \ve{\wt v_{t+\eta}-w_{t+\eta}}_2
&\le e^{-\fc{r}{2\ka}} \sqrt{F(y_{t}=\wt x_t, w_{t}=\wt v_t, x_{t},v_{t})} + 
r^2 \sqrt{\cal E_K}
\label{e:ind-2-term}
\end{align}
where the bound for the first term is from~\eqref{e:Fyw} and 
%comes from Lemma~\ref{l:cont-couple} and 
the bound for the second term comes from Lemma~\ref{l:cont-disc}. This is at most the value of~\eqref{e:ind-2-term} at $r=\eta$ by convexity.
Plugging in the bound on $\sqrt{F(\wt x_t, \wt v_t, x_{t},v_{t})}$ shows~\eqref{e:induct1} for $t+r\in (t,t+\eta]$.
%completes the induction step fo.

Finally, note that~\eqref{e:Fyw} and~\eqref{e:Fxv} give the theorem.
\end{proof}

\begin{lem}\label{l:disc2}
Suppose $\eta\le \rc{8\sqrt 2\ka}$. Suppose that $(x^{(\eta)}_s, v^{(\eta)}_s)$ and $(x_s,v_s)$ are synchronously coupled discrete and continuous processes coinciding at $s=0$.
%Suppose $\eta_1,\eta_2\le \rc{8\sqrt 2\ka}$. Suppose that $(x^{(\eta_j)}_s,v^{(\eta_j)}_s)$ are synchronously coupled discrete processes for $j=1,2$, coinciding at $s=0$. (The coupling is done through the continuous process.) 
%Suppose $T\ge 2$. %Let $\cal E = E_0 + \Dvals$.
If $u\ge \fc{16\ka \sqrt{E_0+2dT}}{\sqrt L}$, then 
%If $u\ge \fc{16\ka (\eta_1+\eta_2)\sqrt{E_0+2 dT}}{\sqrt L}$, then 
%\begin{align}
%\Pj\pa{\ve{x^{(\eta_1)}_T - x^{(\eta_2)}_T}> 8\ka (\eta_1+\eta_2)\sfc{2\cal E}{L}}\le%\ep.
%2\exp\pa{-\fc{\cal E}{32\ga T}}.
\begin{align}
\Pj\pa{\ve{x^{(\eta)}_T - x_T}>a}
&\le \exp\pa{-\fc{a^2}{(64\ka \eta/L)^2}}.
%\Pj\pa{\ve{x^{(\eta_1)}_T - x^{(\eta_2)}_T}>u}
%&\le \exp\pa{-\fc{u^2}{(64\ka (\eta_1+\eta_2)/L)^2}}.
\end{align}
%for $K=\fc{64\ka (\eta_1+\eta_2)}{\sqrt L}$. Thus, 
%Moreover, 
Moreover, if $T\ge 8$, then $\ve{x^{(\eta)}_T - x_T}$ is $\fc{16 \ka \eta\sqrt{E_0+2 dT}}{\sqrt L}$-subgaussian.
%Moreover, if $T\ge 8$, then $\ve{x^{(\eta_1)}_T - x^{(\eta_2)}_T}$ is $\fc{16 \ka (\eta_1+\eta_2)\sqrt{E_0+\ga dT}}{\sqrt L}$-subgaussian.
%$\fc{64\ka (\eta_1+\eta_2)}{\sqrt L}$-subgaussian.
%$K$-subgaussian for 
%\begin{align}
%K&=8\ka (\eta_1+\eta_2) \sqrt{
%\fc{8dT}{L} + \fc{2E_0}L + \fc{16T\log 2}{L^2}
%}.
%\end{align}
\end{lem}
\begin{proof}
By Lemma~\ref{l:bounded-E}, if
$D\ge 2\pa{E_0+2 dT}$, 
then
\begin{align*}
\Pj\pa{
\sup_{0\le t\le T} E_t \ge D
%E_0 + \Dval %2\ga dT + 16u \log \pf{2}{\ep}
}&\le %\ep.
2\exp\pa{-\fc{D}{64 T}}
\end{align*}
If $\sup_{0\le t\le T} E_t <D$, then by Lemma~\ref{l:cont-disc2}, 
%for $j=1,2$,
\begin{align*}
\ve{x^{(\eta)}_T - x_T} &\le  8\ka \eta \sfc{2D}{L}.
%\\
%\ve{x^{(\eta_1)}_T - x_T} &\le  8\ka \eta \sfc{2D}{L}
\end{align*}
%so by the triangle inequality, 
%\begin{align*}
%\ve{x^{(\eta_1)}_T - x^{(\eta_2)}_T} &\le  8\ka (\eta_1+\eta_2) \sfc{2D}{L}
%\end{align*}•
Now take $D=\fc{L u^2}{128 \ka^2 \eta^2}$. We note that the condition for $D\ge 2(E_0+2 dT)$ is equivalent to $u\ge \fc{16\ka \eta\sqrt{E_0+2 dT}}{\sqrt L}$.

The concentration inequality implies that  $\ve{x^{(\eta)}_T - x_T}$ is $K$-subgaussian for $K=\max\bc{\fc{2^6 \ka\eta}{\sqrt L}, 2^4 \ka \eta\sfc{E_0+2 dT}L}$.  The second term is larger since $\sqrt{E_0+2 dT}\ge 4$.
%This follows from coupling with the continuous process (Lemma~\ref{l:cont-disc2}) and using the triangle inequality. For the subgaussian constant, note that
%\begin{align}
%\max\bc{
%2e^{\fc{E_0L}{8T}+\fc{Ld}2-\fc{L^2}{16T}\pf{r}{8\ka (\eta_1+\eta_2)}^2},1
%}\le 
%\max\bc{
%2e^{-\fc{r^2}{K^2}},1
%}.
%\end{align}•
\end{proof}

\subsection{Computing the normalizing constant with MULD}

We are now ready to prove our main theorem, by combining Theorem~\ref{t:muld} with Lemma~\ref{l:prod}. %We proceed as in Theorem~\ref{t:muld}, but use Lemma~\ref{l:prod} as we wish to estimate a product of ratios. 
%There is a technical point that the ratio $g$ is not Lipschitz, as it grows exponentially for large $\ve{x}$; however, because large $x$'s are very unlikely under $\rh$, the expected value of $g$ changes very little if we replace it by a ``clamped" version of $g$ (Lemma~\ref{l:g-tail}).

\begin{proof} %Error from 
~\paragraph{Bias at each temperature.} 
At each temperature we first estimate $\ol r_i$. Choose the step size to be $\eta=O\pa{\rc{\ka}\sfc{\mu_i}d}$. Then the estimate $g(\wt X)$ is $O\pa{\sqrt{d}}$-subgaussian. This takes $\fc{T}{\eta}=\Te\pa{\ka^2 \fc{d}{\mu_i} \log(d)}$ steps. Taking $\Te=O\pa{\log(d) \log\prc{\de_1}}$ samples, we can estimate $\ol r_i$ to within $\fc{\si_i}4$ with probability $\ge 1-\de_1$. Let the estimate be $\wt r_i$.

Now take $r^+=\wt r_i + \pa{\sqrt{2(1+\al)\log \prc{\ep_1}}+\rc4}\si_i$. Then with probability $\ge 1-\de_1$, because $\ep_1\le e^{-1}$,
\begin{align*}
r^+&\in \ol r_i +\pa{\sqrt{2(1+\al)\log \prc{\ep_1}}+\ba{0,\rc 2}}\si_i
\subeq \ol r + \sqrt{(1+\al)\log \prc{\ep_1}}\si_i [\sqrt 2,2].
\end{align*}


\paragraph{Variation at each temperature.}
Let $\ka = \fc{L}{\mu}$. Note that $f_i(x) =\fc{\ve{x}^2}{2\si_i^2} + f(x)$ is $\mu_i = \mu+\rc{\si_i^2}$-strongly convex, $L_i=L_i+\rc{\si_i^2}$-smooth, and has condition number $\fc{L_i}{\mu_i}\le \ka_i$. 

Suppose $\ep_1+\ep_2\le \rc 2$. Let $\wh R_i$ be the estimate at the $i$th temperature, $\wt R_i = \E \wh R_i = \E_{\wt \rh_i}h_i(x)$, and $R_i = \E_{\rh_i}g_i$. Then
$\fc{|\wt R_i-R_i|}{R_i}\le \rc 2$, so $\wt R_i \ge \rc 2 R_i$. 
%If $\wh R_i - \wt R_i$ is $CR_i$-subgaussian, then $\fc{\wh R_i - \wt R_i}{R_i}$ is $2CR_i$-subgaussian.
In order to make $\ve{\wh R - \wt R_i}_{\Psi_2}^2 \le \fc{\ep_3^2R_i^2}{4M}=: \ep_\si^2$ and $|\wt R_i - R_i|\le \fc{\ep_3R_i}{2M} =:\ep_b$, the number of time steps required is
%The number of time steps required to make $\fc{\wh R_i-\wt R_i}{R_i}$ $\ep_\si$-subgaussian, and to make ${|\wt R_i-R_i|}{R_i}\le \ep_b$ is
\begin{align*}
&O\pa{
\ka^2 \sqrt d M \log \pf{d}{\mu_i\ep_b} \pa{\fc{\prc{\si_i}^2 R_i^2}{\ep_\si^2 \mu_i}
+ 
\fc{\prc{\si_i} R_i}{\ep_b \sqrt{\mu_i}}
}
}\\
&=
O\pa{
\ka^2 \sqrt d M \log \pf{d}{\prc{\si_i^2}\ep_3R_i} \pa{\fc{\prc{\si_i}^2 R_i^2}{(\ep_\si R_i)^2 \prc{\si_i^2}}
+ 
\fc{\prc{\si_i} R_i}{(\ep_b R_i) \prc{\si_i}}
}
}
= 
O\pa{\fc{\ka^2 \sqrt d M}{\ep_3^2} \log\pf{d\si_i^2}{\ep_3 R_i} }
\end{align*}
where we substitute $\ep_b$ and $\ep_\si$ and use $\mu_i\ge \rc{\si_i^2}$. 
%Letting $\ep_b=\fc{\ep_3}{\sqrt d}$ and $\ep_\si^2 = \fc{\ep_3^2}{\sqrt d}$, we get that this is $O\pa{\fc{\ka^2 d}{\ep_3^2} \log\pf{d}{m\ep} }$.
\fixme{We also note that $W_2(\rh_i,\wt \rh_i)\le \fc{\ep_b}{2L_{h_i}}$, so $L_{h_i} W_2(\rh_i,\wt \rh_i)\le \fc{\ep_b}2\le \fc{\ep_3R_i}{4}$, and we get $\fc{|\E_{\wt\rh_i}h_i - \E_{\rh_i}g_i|}{|\E_{\rh_i}g_i|}\le \ep_1 + \ep_3$.
}


\end{proof}

\subsection{Subgaussian and subexponential random variables}

We recall a few facts about subgaussian and subexponential random variables.

\begin{df}
For a convex function $\Phi:[0,\iy)\to [0,\iy)$ such that $\fc{\Phi(x)}{x}\to 0$ as $x\to 0$ and $\fc{\Phi(x)}{x}\to \iy$ as $x\to \iy$, and a $\R$-valued random variable $X$, define the Orlicz norm
$$\ve{X}_{\Phi} := \inf\set{0<K<\iy}{\E\ba{\Phi\pf{|X|}{K}}\le 1}.$$ 

Let $\Psi_j (x) = e^{x^j}-1$. If $\ve{X}_{\Psi_1}\le K$, we say $X$ is $K$-subexponential, and if $\ve{X}_{\Psi_2}\le K$, we say $X$ is $K$-subgaussian. We say $X$ is $K$-subexponential or subgaussian around its mean if $X-\E X$ is $K$-subexponential or subgaussian, respectively.
\end{df}
\begin{pr}[\cite{vershynin2018high}]
\label{p:sub}
%Let $X$ be a $\R$-valued random variable.
%For $j\in \{1,2\}$, there exist $C_j,C_j'$ such that following hold.
Let $j\in \{1,2\}$. The following hold. 
\begin{enumerate}
\item There exists $C_j$ such that if $X$ is a $\R$-valued random variable and for all $t>0$, $\Pj(|X|\ge t)\le 2\exp\pa{-\fc{|t|^j}{K^j}}$, then $\ve{X}_{\Psi_j}\le C_j K$. ($C_j = e^{-\fc{j}2}$ works.)
Conversely, there exists $K_j$ such that if $\ve{X}_{\Psi_j}\le K$, then $\Pj(|X|\ge t)\le 2\exp\pa{-\fc{|t|^j}{(K_jK)^j}}$.
\item There exists $C_j'$ such that if $\ve{X}_{\Psi_j}\le K$, then for all $p\ge 1$, $\E[|X|^p]^{\rc p}\le C_j' K p^{\rc{j}}$.
\item There exists $C'$ such that if $X_i$, $1\le i\le N$ are independent mean-0 $\R$-valued random variables, then 
$\ve{\sumo iN X_i}_{\Psi_j}^j \le C' \sumo iN \ve{X_i}_{\Psi_j}^j$. ($C'=\fc{4}{e}$ works.)
\item For a $\R$-valued random variable $X$, $\ve{X}_{\Psi_2}^2 = \ve{X^2}_{\Psi_1}$.
\item (Centering) For a $\R$-valued random variable $X$,  $\ve{X-\E X}_{\Psi_j}\le \ve{X}_{\Psi_j}$. 
\item If $X$ is a $\R^d$-valued random variable and $g$ is $L$-Lipschitz, then $\ve{g(X)-\E g(X)}_{\Psi_j}\le L\ve{\ve{X-\E X}}_{\Psi_j}$. 
\end{enumerate}
\end{pr}

\subsection{Other}
\begin{thm}[{Harg\'e, \cite{harge2004convex}}]\label{thm:harge}
%Suppose that $X\sim N(0,\Si)$ has density $\ga$ and $Y$ has density $p=h\cdot \ga$, with $h$ log-concave. Let $g$ be convex. Then
Suppose the $d$-dimensional gaussian $N(0,\Si)$ has density $\ga$. Let $p=h\cdot \ga$ be a probability density, where $h$ is log-concave. Let $g:\R^d\to \R$ be convex. Then
\begin{align}
\int_{\R^d} g(x-\EE_p x)p(x)\dx &\le \int_{\R^d} g(x)\ga(x)\dx.
\end{align}
\end{thm}



==> stoc.tex <==
% \documentclass[sigconf,screen]{acmart} 

% \usepackage{amsmath,amsbsy,amsfonts,amssymb,dsfont,units}
% \usepackage{amsthm}
% %\usepackage[alphabetic]{amsrefs}
% \usepackage{graphicx}
% %\usepackage{authblk}
% \usepackage{todonotes}
% \usepackage{stmaryrd}
% %\usepackage[margin=1in]{geometry}
% \usepackage[bottom]{footmisc}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
%  \usepackage{microtype}
%  \usepackage{flushend}
%  \usepackage{balance}
 
% \usepackage{caption}

% \usepackage{etoolbox}

% %\usepackage{algorithm}
% %\usepackage{algpseudocode}
% \usepackage{algorithm,algorithmic,mathtools}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \usepackage{color,cases}
% \usepackage{tikz}
% \usetikzlibrary{calc,shapes}
% \usepackage{subfigure}
% %\usepackage[round]{natbib}
% \usepackage{hyperref}

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{thm}[theorem]{Theorem}
% \newtheorem*{thm*}{Theorem}
% %\newtheorem{corollary}{Corollary}[section]
% %\newtheorem{assumption}{Assumption}[section]
% %\newtheorem{lemma}{Lemma}
% %\newtheorem{lem}[lemma]{Lemma}
% %\newtheorem{pr}{Proposition}[section]
% %\newtheorem{proposition}{Proposition}[section]
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{cor}[theorem]{Corollary}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{lem}[theorem]{Lemma}
% \newtheorem*{lem*}{Lemma}
% \newtheorem{pr}[theorem]{Proposition}
% \newtheorem{proposition}[theorem]{Proposition}

% \newtheorem{claim}{Claim}[section]

% \theoremstyle{definition}
% \newtheorem{condition}{Condition}[section]
% %\newtheorem{definition}{Definition}
% %\newtheorem{df}[definition]{Definition}
% %\newtheorem{example}{Example}
% %\theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{rem}[theorem]{Remark}
% \newtheorem*{rem*}{Remark}
% %
%  \newcommand{\IGNORE}[1]{}

% \newcommand{\cites}{\cite}
% %\newcommand{\citep}{\cites}
% %\newcommand{\citet}{\cites}
% %\newcommand{\citealp}{\cites}
% \def\nn{\nonumber}

% %%%%%from other papers
% \newcommand\E{\mathbb{E}}
% \newcommand\EE{\mathbb{E}}

% \newcommand\R{\mathbb{R}}
% \newcommand\RR{\mathbb{R}}

% \newcommand\N{\mathcal{N}}
% \newcommand\cF{\mathcal{F}}
% \def\Pbb{\mathbb{P}}

% \renewcommand\t{{\scriptscriptstyle\top}}
% \DeclareMathOperator{\diag}{diag}
% \DeclareMathOperator{\Astar}{\tilde{A}}
% \DeclareMathOperator{\Bstar}{\tilde{B}}
% \DeclareMathOperator{\Cstar}{\tilde{C}}
% \DeclareMathOperator{\wstar}{\tilde{w}}
% \DeclareMathOperator{\astar}{\tilde{a}}
% \DeclareMathOperator{\bstar}{\tilde{b}}
% \DeclareMathOperator{\cstar}{\tilde{c}}
% \DeclareMathOperator{\var}{Var}

% \newcommand\mc{\mathcal}

% \newcommand{\wb}{\overline}
% \newcommand\wh{\widehat}

% \newcommand\wt{\widetilde}
% \newcommand\eps{\varepsilon}
% \newcommand\veps{\varepsilon}
% \newcommand\h{\hat}

% \newcommand{\Or}{\mathcal{O}}

% \newcommand{\rd}{\mathrm{d}}
% \newcommand{\ud}{\,\mathrm{d}}


% \newcommand{\abs}[1]{\lvert#1\rvert}
% \newcommand{\norm}[1]{\lVert#1\rVert}


% \newcommand\tl{\tilde}
% %\newcommand\bar{\overline}
% \newcommand\inner[1]{\langle #1 \rangle}
% \newcommand\sign{\operatorname{sign}}

% \newcommand\indicator[1]{\ensuremath{\mathbf{1}_{#1}}}

% %\newcommand{\llabel}[1]{{\color{red}#1}\label{#1}}
% \newcommand{\ifstoc}[2]{\iftoggle{stoc}{#1}{#2}}

% \newtoggle{final}
% \togglefalse{final}  %CHANGE WHEN DONE
% \toggletrue{final}
% \newtoggle{arxiv}
% \togglefalse{arxiv}
% \newtoggle{stoc}
% \toggletrue{stoc}
% %\togglefalse{final}
% %\newcommand{\paper}[0]{work}

% \newcommand{\draft}[1]{\iftoggle{final}{}{#1}}
% \newcommand{\revise}[1]{{\draft{\color{blue}}#1}}

% \newcommand{\fixme}[1]{\draft{\color{red}#1}}
% \newcommand{\rgcom}[1]{\draft{\noindent{\textcolor{blue}{Rong: #1}}}}
% \newcommand{\jlcom}[1]{\draft{\noindent{\textcolor{blue}{Jianfeng: #1}}}}
% \newcommand{\hlcom}[1]{\draft{\noindent{\textcolor{purple}{Holden: #1}}}}
% \input{macros_stoc}

% \title{Estimating Normalizing Constants for Log-Concave Distributions: Algorithms and Lower Bounds}

% \author{Rong Ge}
% \affiliation{
% \institution{Duke University}
% \city{Durham}
%  \state{NC}
%  \country{USA}}
% \email{rongge@cs.duke.edu}

% \author{Holden Lee}
% \orcid{0000-0003-3534-8739}
% \affiliation{
% \institution{Duke University}
% \city{Durham}
%  \state{NC}
%  \country{USA}}
% \email{holee@math.duke.edu}

% \author{Jianfeng Lu}
% \affiliation{
% \institution{Duke University}
% \city{Durham}
%  \state{NC}
%  \country{USA}}
% \email{jianfeng@math.duke.edu}
% %\date{November 4, 2019}


% %%% The following is specific to STOC '20 and the paper
% %%% 'Estimating Normalizing Constants for Log-Concave Distributions: Algorithms and Lower Bounds'
% %%% by Rong Ge, Holden Lee, and Jianfeng Lu.
% %%%
% \setcopyright{acmlicensed}
% \acmPrice{15.00}
% \acmDOI{10.1145/3357713.3384289}
% \acmYear{2020}
% \copyrightyear{2020}
% \acmSubmissionID{stoc20main-p365-p}
% \acmISBN{978-1-4503-6979-4/20/06}
% \acmConference[STOC '20]{Proceedings of the 52nd Annual ACM SIGACT Symposium on Theory of Computing}{June 22--26, 2020}{Chicago, IL, USA}
% \acmBooktitle{Proceedings of the 52nd Annual ACM SIGACT Symposium on Theory of Computing (STOC '20), June 22--26, 2020, Chicago, IL, USA}


% \begin{CCSXML}
% <ccs2012>
% <concept>
% <concept_id>10003752.10010070.10010071.10010077</concept_id>
% <concept_desc>Theory of computation~Bayesian analysis</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10003752.10010061.10010065</concept_id>
% <concept_desc>Theory of computation~Random walks and Markov chains</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10003752.10003809.10003636.10003815</concept_id>
% <concept_desc>Theory of computation~Numeric approximation algorithms</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10002950.10003648.10003670.10003677.10003680</concept_id>
% <concept_desc>Mathematics of computing~Simulated annealing</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10002950.10003648.10003649.10003656</concept_id>
% <concept_desc>Mathematics of computing~Stochastic differential equations</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% <concept>
% <concept_id>10002950.10003648.10003700.10003701</concept_id>
% <concept_desc>Mathematics of computing~Markov processes</concept_desc>
% <concept_significance>500</concept_significance>
% </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Theory of computation~Bayesian analysis}
% \ccsdesc[500]{Theory of computation~Random walks and Markov chains}
% \ccsdesc[500]{Theory of computation~Numeric approximation algorithms}
% \ccsdesc[500]{Theory of computation~Bayesian analysis}
% \ccsdesc[500]{Mathematics of computing~Simulated annealing}
% \ccsdesc[500]{Mathematics of computing~Stochastic differential equations}
% \ccsdesc[500]{Mathematics of computing~Markov processes}




% \keywords{Langevin Monte Carlo, multilevel Monte Carlo, normalizing constant, partition function, log-concave distribution, sampling algorithm}

% %\includeonly{intro,prelim,upperbound,multilevel-main,lowerbound}
% %\let\clearpage\relax

% \begin{document}
% \begin{abstract}
%     Estimating the normalizing constant of an unnormalized probability distribution has important applications in computer science, statistical physics, machine learning, and statistics. In this work, we consider the problem of estimating the normalizing constant $Z=\int_{\mathbb{R}^d} e^{-f(x)}\,\mathrm{d}x$ to within a  multiplication factor of $1 \pm \varepsilon$ for a $\mu$-strongly convex and $L$-smooth function $f$, given query access to $f(x)$ and $\nabla f(x)$.
%     We give both algorithms and lowerbounds for this problem. Using an annealing algorithm combined with a multilevel Monte Carlo method based on underdamped Langevin dynamics, we show that     $\widetilde{\mathcal{O}}\Bigl(\frac{d^{4/3}\kappa + d^{7/6}\kappa^{7/6}}{\varepsilon^2}\Bigr)$ 
%     queries to $\nabla f$ are sufficient, where $\kappa= L / \mu$ is the condition number. Moreover, we provide an information theoretic lowerbound, showing that at least $\frac{d^{1-o(1)}}{\varepsilon^{2-o(1)}}$ queries are necessary. This provides a first nontrivial lowerbound for the problem. 
% \end{abstract}

% {\sloppy
% \maketitle
% }
% %\pagebreak

% \input{intro}

% \input{prelim}



% \input{upperbound}

% \input{multilevel-main}

% \input{lowerbound}

% %\input{alt_upperbound.tex}

% \input{conclusion}


% \section*{Acknowledgements}

% HL would like to thank Oren Mangoubi for introducing multilevel methods. RG and HL would like to thank Ruoqi Shen for explaining the paper~\cite{shen2019randomized}. RG acknowledges funding from NSF CCF-1704656, NSF CCF-1845171 (CAREER), Sloan Fellowship and Google Faculty Research Award. Part of the work was done while RG was visiting the Institute for Advanced Study. The work of JL is supported in part by National Science Foundation via grants DMS-1454939 and CCF-1934964. 

% %\bibliographystyle{amsxport}
% %\newpage
% %\vspace{0in}
% \bibliographystyle{unsrt}
% \balance
% \bibliography{sampling}
% % \appendix
% % \newpage

% % \input{annealing-proof}
% % \input{mala-proof}
% % \input{multilevel}
% % \input{lowerbound-proof}
% % \input{quadrature}
% % \input{appendix}
% \end{document}

